Auto-X3D: Ultra-Efficient Video Understanding via Finer-Grained Neural Architecture Search

Efficient video architecture is the key to deploying video recognition systems on devices with limited computing resources. Unfortunately, existing video architectures are often computationally intensive and not suitable for such applications. The recent X3D work presents a new family of efficient video models by expanding a hand-crafted image architecture along multiple axes, such as space, time, width, and depth. Although operating in a conceptually large space, X3D searches one axis at a time, and merely explored a small set of 30 architectures in total, which does not sufficiently explore the space. This paper bypasses existing 2D architectures, and directly searched for 3D architectures in a fine-grained space, where block type, filter number, expansion ratio and attention block are jointly searched. A probabilistic neural architecture search method is adopted to efficiently search in such a large space. Evaluations on Kinetics and Something-Something-V2 benchmarks confirm our AutoX3D models outperform existing ones in accuracy up to 1.3% under similar FLOPs, and reduce the computational cost up to x1.74 when reaching similar performance.

==> WACV AutoX3D (camera ready)/tex/0_abstract.tex <==
\begin{abstract}

Efficient video architecture is the key to deploying video recognition systems on devices with limited computing resources. Unfortunately, existing video architectures are often computationally intensive and not suitable for such applications. The recent X3D work presents a new family of efficient video models by expanding a hand-crafted image architecture along multiple axes, such as space, time, width, and depth. Although operating in a conceptually large space, X3D searches one axis at a time, and merely explored a small set of 30 architectures in total, which does not sufficiently explore the space. This paper bypasses existing 2D architectures, and directly searched for 3D architectures in a fine-grained space, where \textit{block type, filter number, expansion ratio} and {attention block} are jointly searched. A probabilistic neural architecture search method is adopted to efficiently search in such a large space.   
Evaluations on Kinetics and Something-Something-V2 benchmarks confirm our \autoxthreed models outperform existing ones in accuracy up to \textbf{1.3}\% under similar FLOPs, and reduce the computational cost up to $\times$\textbf{1.74} when reaching similar performance. 
% Code will be publicly available. 

\end{abstract}

==> WACV AutoX3D (camera ready)/tex/1_intro.tex <==
\section{Introduction}

Video models are arguably living in a much larger design space than image models, as they are expected to abstract information in both spatial- and temporal dimensions, which requires a larger set of layer types and more complicated arrangements of the layers. However, many existing video models are simply built on top of image models, which are tailored to process video by applying image models to individual/a stack of frames (e.g. two-stream network~\cite{twostreamconvnet}), replacing 2D- with 3D convolution (e.g. C3D~\cite{c3d}, I3D~\cite{i3d}, S3D~\cite{s3d}, CSN~\cite{csn}), or adding temporal convolution (e.g. R(2+1)D~\cite{r2plus1}). Such an image-to-video design process has served us as a fast path to build video architectures, but may also limit our exploration of the video architectures. On the other side, to design video architectures from scratch, one needs to take into account many more factors, than that of image recognition models. For example, one has to not only extend the inputs, features, and/or filter kernels into the temporal axis \cite{i3d}, but also strike a balance over many factors, such as the depth (number of layers), width (filter number), and spatial resolution, to achieve a good Accuracy-To-Complexity (ATC) trade-off \cite{2019efficientnet}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/AutoX3D_benchmark.png}
    % \vspace{-5pt}
    \caption{\textbf{Main results on Kinetics-400}. Compared to other SOTA models, the proposed AutoX3D network series achieve better Accuracy-To-Complexity (ATC) trade-off.}
    \label{fig:atc_curve}
    % \vspace{-5pt}
\end{figure}

Recently, machine-designed architectures by Neural Architecture Search (NAS) have surpassed the human-designed ones for image recognition~\cite{2019AmoebaNet, pham2018efficient, 2019efficientnet, bignas}. For video action recognition, the latest work X3D~\cite{x3d} placed a new milestone in this line: it progressively expanded a hand-crafted 2D architecture into 3D spatial-temporal ones, by expanding along multiple axes, including space, time, width, and depth. As the joint search space of all axes is extremely large, X3D only searches over one axis at a time, progressively expanding the architectures to meet the target complexity. Although competitive ATC trade-off is achieved, those architectures are searched after only exploring 30 architectures in the space, which includes a total of 3,780 architectures. \textit{Can we search video architectures with better ATC if the design space is more sufficiently explored?} 

Moreover, X3D models still conform to many manual design choices in the hand-crafted 2D architecture based on MobileNet~\cite{2018mobilenetv2}. For example, the temporal-spatial kernel size is fixed to be $3\times3^2$ for depthwise convolution in the 3D MBConv (Mobile Inverted Bottleneck Conv) building block, the expansion rate is fixed to be $2.25$, and all blocks in the same stage chooses the same number of filters while the difference in the number of filters between blocks from neighboring stages is always $2\times$. For the model architecture, X3D only explores to uniformly expand the number of filters and number of blocks to change the model complexity. \textit{Can we go beyond hand-crafted 2D architectures, and directly search for 3D architectures while allowing different architectures in individual building blocks?}

This paper aims to address those questions, and takes steps further towards the direction of \textit{efficient video recognition }. The goal is fundamentally challenging as it requires us to rethink the design space of the video architecture, relax many constraints which are made to facilitate manual exploration, and more aggressively explore the design space.

To this end, this paper directly searches for efficient video architecture, leading to our work of \textbf{\autoxthreed}. Different from X3D which ignores the variations of the block types and only uniformly expands the channels, we introduce a fine-grained search space for efficient video models, by including more efficient operations. Unlike the conventional differentiable NAS (e.g. DARTS~\cite{2018darts}), which repeatedly stacks the cells of the same structure in the network, our search allows independent blocks at different layers. 
In our fine-grained space, we jointly search for the block types, filter numbers, expansion ratio, and attention blocks, substantially surpassing those in previous work on image NAS~\cite{2018darts, 2019AmoebaNet, 2019nasnet, fbnet} and video NAS~\cite{x3d, assemblenet, assemblenet, assemblenet++}. 
To support fast search, we adopt the probabilistic differentiable NAS (PARSEC)~\cite{2019pnas} as the basic search algorithm, which requires much less memory footprint than conventional DNAS (e.g. DARTS~\cite{2018darts}). Furthermore, we extend it to support the joint search among different factors (depth, channel, expansion ratio etc.). 
For better sample efficiency in our search space, we introduce the fairness-aware channel selection strategy into the probabilistic search algorithm, which enables a more stable, accurate, and scalable search framework for our task. 

To summarize, we view the contributions as following.
% \vspace{-5pt}
\begin{itemize}[leftmargin=*]
\item A fine-grained design space for efficient video recognition is proposed, to jointly search the block types, filter numbers, expansion ratio, and attention blocks.
\item A family of efficient \autoxthreed models, which are directly searched without any architecture surrogate or the use of hand-crafted image architecture, are presented. Their architectures are distinctive from hand-crafted models, and provide new insights of designing video architectures.
\item Extensive evaluations on Kinetics~\cite{kay2017kinetics} and Something-Something~\cite{sthsth} benchmarks confirm our \autoxthreed models achieve significantly better accuracy-to-complexity trade-off than other existing models.

\end{itemize}


==> WACV AutoX3D (camera ready)/tex/2_related_work.tex <==
\section{Related Work}

\subsection{Video Architecture Design}

%Video sequences contain an extra temporal dimension than images ($C$$\times$$T$$\times$$H$$\times$$W$) compared to image ($C$$\times$$H$$\times$$W$). Therefore, 
Early video models are built on top of image ones. As the name implies, Two-Stream Network \cite{twostreamconvnet} uses two streams of image architectures to process single-frame and multi-frame optical flow inputs, respectively. To capture temporal feature, R(2+1)D~\cite{r2plus1} adds 1D temporal convolution to the 2D ResNet model while I3D~\cite{i3d} replaces 2D convolution with more expensive 3D convolution. To model long-range temporal relations, \cite{yue2015beyond,donahue2015long} runs LSTMs on top of image features extracted from video frames, while \cite{nonlocal_block} uses non-local blocks. Those video architectures are computationally heavy, and not suitable to be deployed on devices with limited computing power.

Due to the prevalence of mobile devices, designing efficient video architectures has become an increasingly important task. Efficient blocks, such as Temporal Shift module~\cite{tsm} and Video Shuffling module~\cite{ma2019learning}, are proposed to capture the temporal dynamics at low cost. More fine-grained adaptation of 2D models is also proposed. For example, in~\cite{s3d} it reports for I3D backbone, top-heavy modeling achieves better ATC trade-off by placing expensive 3D convolutions in the top layers only. However, such adaptation is not effective for ResNet backbone \cite{r2plus1}, highlighting the limitation of manually designed video architectures. Recently, search-based video architecture design, such as Tiny Video Network~\cite{piergiovanni2019tiny} and X3D~\cite{x3d}, has made significant progress towards efficient video architecture. In particular, X3D presents new insights for turning a 2D architecture into 3D one by progressively expanding it along multiple axes, such as width, depth, and time. Different from X3D, we completely search video architecture from scratch in a more fine-grained space, and demonstrate the discovered architectures can squeeze out more gain in terms of efficiency and accuracy. 


\subsection{Neural Architecture Search Methods}

Neural architecture search (NAS) aims to replace the laborious human design of network architectures, as well as towards more efficient ones~\cite{2019Mnasnet}. The conventional evolution or reinforcement learning-based search methods are slow and take thousands of GPU days. For example, searching an image model for CIFAR-10 and ImageNet
required 2000 GPU days of reinforcement learning (RL)~\cite{zoph2016neural} or 3150 GPU days of evolution~\cite{2019AmoebaNet}. ENAS~\cite{pham2018efficient} introduced a parameter-sharing strategy to reduce the search time. Recent differentiable NAS (DNAS) methods~\cite{2018darts} introduced the softmax-based continuous relaxation of the architecture representation, allowing efficient search using gradient descent. However, they compute features for all layer choices, and uses much more memory than standalone model training. The probabilistic version of DNAS, such as PARSEC~\cite{2019pnas}, describes the population of architectures in the design space by a distribution, and only requires to sample one architecture at a time, which uses memory only as much as in the standalone model training. In this work, we employ PARSEC as the search procedure to search efficient video architectures in our fine-grained search space due to its low memory footprint and fast search efficiency.


\subsection{Neural Architecture Design Space}
The success of searching efficient models depends not only on the efficiency of the search method, but also on the prescription of the architecture design space. In~\cite{radosavovic2019network}, a new comparison paradigm is proposed to compare different design spaces. NASNet~\cite{2019nasnet} proposed a design space of a cell which is a directed acyclic graph. Only the connectivity between graph nodes and the operator type on each graph edge is searched. The final model is obtained by stacking cells with the same architecture. Similarly, DARTS~\cite{2018darts} also only searches the cell architecture, and repeats cells to obtain the final model. Although sharing the architectures across cells can reduce the size of model design space and simplify the search, it can be detrimental to video architecture design. Recent hand-crafted video models, such as S3D~\cite{s3d} and SlowFast~\cite{slowfast}, only use expensive 3D convolution in the top layers to improve the ATC trade-offs, while leaving convolutions in the bottom layers to be 2D. Other design choices, such as the building block type and filter number, are still manually chosen and often uniform. To search for efficient video models, we relax such hard-coded constraints, allow individual building blocks to have separate architectures and filter numbers.


 

==> WACV AutoX3D (camera ready)/tex/3_1_building_block.tex <==


\subsection{Nonuniform Block Micro-Architecture}
In X3D models, the 3D MBConv building block always consists of a conv$1\times1$ layer to expand the filter number, a depthwise convolution layer of kernel size $3\times3^2$ to convolve with spatial features, and another conv$1\times1$ layer to shrink the filter number in the final output feature. Depthwise convolution with kernel $3\times3^2$ is more expensive than that with a 2D kernel of size $1\times3^2$, and such choice of uniform building block micro-architecture is sub-optimal to achieve good ATC. Many prior works~\cite{r2plus1, s3d} have examined the progressively varying temporal-spatial feature patterns along with the model depth. For example, S3D~\cite{s3d} work has shown employing 3D convolution at bottom layers (close to input) is less cost-effective than using it at top layers (close to final prediction). On the other side, other convolution kernel sizes, such as $1\times5^2$ and $3\times5^2$, are not yet explored in hand-crafted models due to a large number of different combinations of spatial-temporal kernel size. In \autoxthreed design space, we consider 3D MBConv block with a different spatial-temporal kernel size in depthwise convolution as a separate block micro-architecture.

% Moreover, the recently proposed Temporal Shift Module (TSM)~\cite{tsm} is an efficient module which only shifts the data along the temporal direction with zero FLOPS but is capable of capturing temporal signals. TSM module can be inserted into the 3D MBConv block at the beginning. We consider the 3D MBConv block with a TSM module inside it as a separate micro-architecture.

In Table~\ref{tab:mbconv3d_micro_arch}, we present the choices of the 3D MBConv block micro-architectures in our design space.

\begin{table}[t]
% \vspace{-0.6cm}
\centering
% \small
% \tiny
% \scriptsize
\resizebox{0.3\linewidth}{!}{

  \begin{tabular}{c|cc}
  \toprule
    Type & Kernel  \\
    \specialrule{.1em}{.1em}{.1em}   

    t1\_s3 & $1\times3^2$  \\   
    t1\_s5 & $1\times5^2$ \\  
    t3\_s3 & $3\times3^2$ \\   
    t3\_s5 & $3\times5^2$ \\
    t5\_s3 & $5\times3^2$  \\   
    t5\_s5 & $5\times5^2$ \\
    % t1\_s3\_tsm & $1\times3^2$ & $\checkmark$   \\
    % t1\_s5\_tsm & $1\times5^2$ & $\checkmark$    \\
    \bottomrule
% \specialrule{.1em}{.05em}{.05em}

  \end{tabular}
}
% \vspace{-5pt}
\caption{\textbf{The choices of MBConv3D block micro architecture in our space.}}
\label{tab:mbconv3d_micro_arch}
% \vspace{-8pt}
\end{table}


==> WACV AutoX3D (camera ready)/tex/3_2_filter_number.tex <==
\subsection{Searchable Filter Number}

The choices of the filter number in the building blocks of the hand-crafted models often follow simple heuristics. For example, in I3D~\cite{i3d}, S3D~\cite{s3d}, R(2+1)D~\cite{r2plus1}, and X3D~\cite{x3d} models, all of which have 4 stages and each stage has multiple building blocks, the filter number of the output feature from the building blocks is fixed within the stage, and is doubled in the next stage. The principle of this heuristic choice is originally from 2D ResNet work~\cite{resnet}, whereby doubling the filter number when the spatial resolution of the 2D feature map is reduced by half in the next stage, all building blocks use a similar amount of FLOPS and the compute of the overall model is evenly distributed to the building blocks. 

However, this principle does not hold for 3D video models, as the 3D feature map has both temporal- and spatial-resolution, and often only the spatial-resolution is reduced by half in the next stage while the temporal resolution is not reduced for achieving high recognition performance. For example, in SlowFast~\cite{slowfast} and X3D~\cite{x3d} models, the temporal resolution is not reduced in all 4 stages.

Moreover, the choice of evenly distributing computation to all building blocks is quite ad-hoc. In our design space, we do not manually prescribe the filter number for the building blocks. Instead, we design a separate range of filter number choices for individual building blocks in the model, and even allow building blocks in the same stage to have different filter numbers. As the choices of filter number have a large impact on both the recognition performance and model computational cost, our flexible design and fine-grained choices allow the search methods to discover architectures with a better ATC trade-off.

The choices of filter numbers for individual building blocks are shown as part of the macro-architecture of our design space in Table~\ref{tab:macro-arch}.

==> WACV AutoX3D (camera ready)/tex/3_3_expansion_rate.tex <==

\subsection{Nonuniform Expansion Rate}
In MBConv block, a conv$1\times1$ layer is used to expand the filter number, and the expansion rate decides the channel number of the feature map where the following depthwise convolution will operate on. For simplicity, a uniform choice of the expansion rate is often chosen by the hand-crafted models. For example, in the original MobileNet family of models~\cite{2018mobilenetv2, mobilenetv3}, all MBConv blocks use the expansion rate 6 while in X3D models~\cite{x3d}, the expansion rate is always 2.25. The uniform choice of the expansion rate ignores the variations of feature representation needed at different model depths, and we hypothesize it leads to sub-optimal architectures. 

In our \autoxthreed design space, we predefine a wide range of choices for the expansion ratio in individual building blocks, and allow different choices are chosen by the building blocks. The choices of the expansion ratio can be seen in the macro-architecture of our design space in Table~\ref{tab:macro-arch}.


==> WACV AutoX3D (camera ready)/tex/3_4_attention_block.tex <==
\begin{table}[!t]
\centering
\centering
{\small
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{1.2mm}{
    \begin{tabular}{lcccccc}
    \toprule
    % 24$\times$$T$$\times$128^{2}
    Max Input & Block & \multirow{2}{*}{Expansion} & \multirow{2}{*}{Channel} & \multirow{2}{*}{Number} & Spatial & Att.   \\
    $C\times T \times S^2$ & Type &  &  &  &  Stride & Block \\
  \specialrule{.15em}{.1em}{.1em}      
    3$\times$$13$$\times$ $160^{2}$ & data & 1 & 24 & 1 & 1 & -\\ \midrule
    3$\times$$13$$\times80^{2}$ & 1$\times3^{2}$ & 1 & 24 & 1 & 2 & -\\ \midrule
    28$\times$$13$$\times$ $40^{2}$ &  TBS  &  \multirow{10}{*}{ 1.5 $\sim$  6.0, 0.75 }   & 12 $\sim$  28, 4 & 1 & 2  & TBS \\
    28$\times$$13$$\times$ $40^{2}$ & TBS &  & 12 $\sim$ 28, 4 & 2 & 1 & TBS \\
    64$\times$$13$$\times$ $20^{2}$ & TBS &  & 24 $\sim$ 64, 8 & 2 & 2 & TBS \\
    64$\times$$13$$\times$ $20^{2}$ & TBS &  & 24 $\sim$ 64, 8 & 3 & 1 & TBS \\
    132$\times$$13$$\times$ $10^{2}$ & TBS &  & 48 $\sim$ 132, 12 & 2 & 2 & TBS \\
    132$\times$$13$$\times$ $10^{2}$ & TBS &  & 48 $\sim$ 132, 12 & 3 & 1 & TBS \\
    132$\times$$13$$\times$ $10^{2}$ & TBS &  & 48 $\sim$ 132, 12 & 3 & 1 & TBS \\
    132$\times$$13$$\times$ $10^{2}$ & TBS &  & 48 $\sim$ 132, 12 & 3 & 1 & TBS \\
    264$\times$$13$$\times$ $5^{2}$ & TBS &  & 96 $\sim$ 264, 24 & 2 & 2 & TBS \\
    264$\times$$13$$\times$ $5^{2}$ & TBS &  & 96 $\sim$ 264, 24 & 2 & 1 & TBS \\
    264$\times$$13$$\times$ $5^{2}$ & TBS &  & 96 $\sim$ 264, 24 & 3 & 1 & TBS \\
    % \midrule
    \midrule
    432 & pool & - & 432 & 1 & - & - \\ \hline
    2048 & fc & - & 2048 & 1 & - & -\\
    \bottomrule
    \end{tabular}
    }
  }
}
% \vspace{-5pt}
\caption{\textbf{The macro-architecture of our \autoxthreed design space. ``TBS'' means the operators that are to be searched.}  }
\label{tab:macro-arch}
% \vspace{-10pt}
\end{table}

\subsection{Searchable Attention Block}
\label{sec:attention_block_variable}

Attention blocks, such as Nonlocal-~\cite{nonlocal_block} and GloRe block~\cite{glore}, can be easily plugged into the backbone model for improving the performance. One can choose to insert more than one such blocks at different layers of the backbone. For example, in the GloRe work~\cite{glore}, for ResNet-50 backbone, it chooses to insert 3 GloRe blocks at Res4 stage for achieving a large gain in accuracy. Since modern deep models often contain dozens of layers and we can insert the attention block after any layer, a manual exhaustive exploration for selecting the best subset of layers to insert attention blocks is almost intractable. In our design space, we view the insertion of the attention block as a search problem, and define a set of choices of the attention block below to search the inserted position.

\noindent{\textbf{Pass through.}} The feature will simply pass through the block without any computation. In practice, it represents no attention block placed here.
% This feature will simply pass through the attention block without any modification.

\noindent{\textbf{GloRe.}} The original GloRe block, which includes a feature projection module, a graph convolution network (GCN) module, and an inverse feature projection module. The feature projection module projects spatial features from the coordinate space to the interaction space by aggregating spatial features with attention. The GCN module reasons over the projected features nodes in the interaction space. Finally, the inverse projection module re-projects the feature nodes back into the coordinate space.
%(Fig \textcolor{red}{TBD}, (b)).

% \noindent{\textbf{Dual-GCN GloRe.}} Different from vanilla GloRe, we stack two GCN modules between the feature projection and inverse feature projection module to increase its capacity of reasoning over the features nodes in the interaction space.

% The choices of attention blocks are also shown in Fig. \ref{fig:design_space}, we set possible inserting position for attention block after each MBConv3D group. Therefore, the maximum number of attention block could be 10 while the minimum is zero, representing that no attention block is picked in search process.

==> WACV AutoX3D (camera ready)/tex/3_5_overall_design_space.tex <==

\subsection{Final \autoxthreed Design Space}

The final design space is illustrated in Figure~\ref{fig:design_space}. In Table~\ref{tab:macro-arch}, we prescribe a video macro-architecture, which mainly consists of a stack of 3D MBConv building blocks. We organize the blocks by groups, and blocks in each group share the same design choices. For each group, we search the micro-architecture, filter number, the expansion rate, and the type of attention block which will be inserted after each group. We allow the block groups to have different choices along those design axes.  In total, our design space contains $2\times10^{32}$ different video architectures, and represents a fine-grained space at a scale that has not been explored before. 

==> WACV AutoX3D (camera ready)/tex/3_design_space.tex <==
\section{\autoxthreed Design Space}
\label{sec:design_space}

In this section, we introduce the design space of \autoxthreed architectures. We define a model as a stack of building blocks, and choose to use the 3D version of Mobile Inverted Bottleneck Conv block (MBConv) from MobileNetV2~\cite{2018mobilenetv2} as our building block. The original MBConv block is proven to be more efficient than the ResNet building block~\cite{resnet} in prior work~\cite{2018mobilenetv2, mobilenetv3} and its 3D version is suitable for building efficient video architectures. Unlike X3D models~\cite{x3d}, in our space, the design of the video architecture is more flexible in the following aspects.

\begin{figure*}[t!]
% \vspace{-0.2cm}
   \centering
   \includegraphics[width=0.95\textwidth]{figs/pipeline.pdf} 
% \vspace{-5pt}
   \caption{\textbf{The macro-architecture of \autoxthreed design space.}}
   \label{fig:design_space}
% \vspace{-5pt}
\end{figure*}


\input{tex/3_1_building_block}

\input{tex/3_2_filter_number}

\input{tex/3_3_expansion_rate}

\input{tex/3_4_attention_block}

\input{tex/3_5_overall_design_space}



==> WACV AutoX3D (camera ready)/tex/4_search_method.tex <==
\section{Search Method}

\subsection{Probabilistic-based Architecture Search}
As video models commonly require larger computation resources than image, directly applying the original differentiable NAS becomes unpractical. Here we adopt the PARSEC~\cite{2019pnas} approach, a probabilistic version of the differentiable NAS method, to guide our search procedure. Compared to DARTS \cite{2018darts}, it only requires much memory as is needed to train a single architecture from our search space. This is because of a memory-efficient sampling procedure as we
learn a probability distribution over high-performing neural network architectures. Here we define a unique discrete architecture as $A$, which is sampled from a prior distribution $ P(A|\pmb{\alpha})$. Architecture parameters $\pmb{\alpha}$ denote the probabilities of choosing different operations. The goal of PARSEC is to optimize the architecture parameter $\pmb{\alpha}$, in order to maximize the architecture accuracy. Concretely, for video recognition where we have video samples $\mathbf{X}$ and labels $\mathbf{y}$, probabilistic NAS can be formulated as optimizing the continuous architecture parameters $\alpha$ via an empirical Bayes Monte Carlo procedure~\cite{rasmussen2003bayesian}
% \vspace{-0.2cm}
\begin{equation}
\begin{split}
P(\mathbf{y} | \mathbf{X},   \mathbf{\omega}, \alpha ) & = \int P(\mathbf{y} | \mathbf{X}, \mathbf{\omega}, A) P(A|\pmb{\alpha}) \textup{d}A \\
& \approx \frac{1}{K} \sum_{k} P(\mathbf{y} | \mathbf{X}, \mathbf{\omega}, A_{k}),
\end{split}
\end{equation}
where $\omega$ denotes the model weights. The continuous integral of data likelihood is approximated by sampling $K$ architectures and averaging the data likelihoods from them. We can jointly optimize architecture parameters $\pmb{\alpha}$ and model weights $\mathbf{\omega}$ by estimating gradients $\nabla _{\alpha}\;\textup{log}\;P(\mathbf{y}|\mathbf{X}, \omega, \pmb{\alpha} )$ and $\nabla _{w} \;\textup{log}\;P(\mathbf{y}|\mathbf{X}, \omega, \pmb{\alpha})$ through the sampled architectures. Typically, the number of sampled architecture $K$ is set to 13, which is sufficient to search for a good architecture empirically, according to our preliminary experiments.

To target at efficient architecture discovering, we rebuild PARSEC to support cost-aware search that aiming to not only finding the best performance architecture but also under determined FLOPs constraint. We achieve this goal by adding another cost-aware hinge loss term to the original loss function. Given an architecture $A_{k}$, the cost-aware loss term $c$ can be written as:
\begin{equation}
\label{eq:cost}
    c(A_{k}) = \frac{1}{T} \max(FLOPs(A_{k})-T, 0),
\end{equation}
where $T$ is our target FLOPs.
All the search variables are jointly searched. %More details about search method can be found in our supplement.

\subsection{Fair Channel Selection}
\label{sec:fair_channel_selection}
\begin{figure*}[t!]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
 \includegraphics[width=\linewidth]{figs/Channel_Selection.pdf}
\end{center}
% \vspace{-10pt}
  \caption{\textbf{Illustration of fairness-aware channel search}, using five channel parts for example. Where $p_i$ is the initial probability of each filter and $g_{i}$ represent the architecture weight of each candidates. We only activate one candidates in the forward pass. All channel candidates share weight from the original filters. For unfair channel selection, the small probability one gets fewer chance to update the corresponding filter compared to large probability one.}
\label{fig:fair}
% \vspace{-10pt}
\end{figure*}

An important pitfall we found during channel search is the \textit{unfairness} for the chances of candidate channels being selected. We show an example in Figure~\ref{fig:fair}: on the left, when splitting the super kernel into $N$ parts ($N$ denotes the channel space size, with $N$ = 5 in the figure just as an example) in the default order, the bottom part will be shared with all channel candidates and therefore always be updated. Meanwhile, the higher bottoms have fewer chances to be updated, with the top one only receiving sparse updates of 1/$N$ probability. That unfairness often leads to the supernet training collapsing onto the most frequently updated channel(s) (e.g. the bottom one), and mislead the architecture selection to sub-optimal performance. To tackle this issue, we propose to \textit{select channels with fairness}, i.e., the assignment of channel candidates shall ensure the chance of selecting/updating each super kernel part to be as equal as possible. Figure~\ref{fig:fair} right displays the fairness-aware selection pattern for $N = 5$, where each part now has the equal chance of 3/5 to be selected and updated. A more general discussion on how to design such fair patterns for different $N$s can be found in the supplement. 




==> WACV AutoX3D (camera ready)/tex/5_1_implementations.tex <==

\subsection{Implementation Details}
\subsubsection{Datasets}

We adopt two benchmarks of video action recognition in the experiments, including Kinetics~\cite{kay2017kinetics} and Something-Something-V2~\cite{sthsth}.

\noindent{\textbf{Kinetics~\cite{kay2017kinetics}}}. Kinetics-400 is a large-scale dataset that contains 400 action classes with 240K training examples and 20K validation examples. To accelerate searching, we adopt Mini-Kinetic200~\cite{xie2018rethinking} as our searching dataset, which is a subset of Kinetics-400 containing 200 classes of videos. As for the evaluation of the searched architecture, we use the full standard Kinetics-400 dataset for training and testing.

% zhicheng: add a dummy box to take the space which is expected to include k400 details
% \begin{solutionorbox}
% \vspace{2cm}
% \end{solutionorbox}

\noindent{\textbf{Something-Something-V2}}.  Something-something-V2 dataset contains 108k videos with 174 classes of diverse actions, while each video lasting between 2 to 6 seconds. Different from Kinetics\cite{kay2017kinetics}, the video sequence in something-something is more temporal related, as it focuses on humans performing predefined basic actions with different objects. Therefore, this dataset serves as a suitable benchmark to evaluate the effectiveness of temporal modeling. %We adopt the new released version Something-Something-V2 in the experiments.

% zhicheng: add a dummy box to take the space which is expected to include sth-sth-v2 details
% \begin{solutionorbox}
% \vspace{2cm}
% \end{solutionorbox}

\subsubsection{Search and Derivation Setting}
\noindent{\textbf{Architecture Search}} We implement PARSEC~\cite{2019pnas} in PyTorch, and use 64 Nvidia V100 GPUs to search architectures on Mini-Kinetics-200. By default, we use the input video clip of size $T\times S^2 = 13\times160^2$ with a spatial scale jittering range of [182, 228], and set the target FLOPS to $2G$ FLOPS, which is on par with the FLOPS of X3D-S model. We adopt Adam with 0.02 learning rate and 0 weight decay to optimize the architecture weights. SGD is adopted to update the supernet's parameters with a learning rate of 0.6, 0.9 momentum, and 5e-5 weight decay. The total search process takes 600 epoches with 3 days. 

\noindent{\textbf{Architecture Training}} We evaluate the searched architectures by using the open-source ClassyVision~\cite{classyvision} framework to train them from scratch on the benchmarks. We use 64 Nvidia V100 GPUs in the experiments. We adopt SGD with 0.9 momentum and 5e-5 weight decay. The learning rate is set to 0.4 following the half-period cosine decaying strategy and mini-batch size is 8 clips per GPU. The whole training process takes 300 epochs while we use linear warm-up strategy \cite{goyal2017accurate} for the first 34 epochs. 
% Moreover, we set SE block\cite{2018senet} and dropout of 0.5 for all architectures. 
Dropout is adopted at the head of the network with the probability of 0.5.  We also apply AutoAugment~\cite{autoaugment} on each frame of input video clip. The data pre-processing part is the same as the searching part. More training detials are illustrated in the supplement.
% \textcolor{red}{On Something-Something-V2, we use the pretrained model weights on Kinetics-400 for initialization. The model is finetuned for 60 epochs, with learning rate 0.6. Other settings are identical to those in the training on Kinetics-400.}
% More training details can be found in our supplement. %

\subsubsection{Architecture Evaluation}
To be comparable with previous work, we mainly follow the evaluation setting of X3D~\cite{x3d}. We evaluate the searched architecture on the validation set. We by default adopt 30-views evaluation, unless specifically stated. Concretely, in 30-views evaluation, 10 clips are uniformly sampled temporally from each video first. Each clip is cropped out using LeftCenterRight cropping strategy~\cite{x3d}, which covers the longer axis of the original clip. The final prediction of a video is obtained by averaging the predictions for all corps of each clip. More details can be found in our supplement.

==> WACV AutoX3D (camera ready)/tex/5_2_ablation.tex <==

\subsection{Ablation Study}
\subsubsection{Searching for Attention Block}
\begin{table}[t!]
\centering
% \small
% \tiny
% \scriptsize
\resizebox{\linewidth}{!}{

  \begin{tabular}{c|cccc|c|c|c}
  \toprule
     \multirow{2}{*}{Model} &  \multicolumn{4}{c|}{Attention location}  & Params & FLOPS & \multicolumn{1}{c}{Accuracy ($\%$)} \\
    & S1 & S2 & S3 & S4 & (M) & (G) & Top-1 \\
    \specialrule{.1em}{.1em}{.1em}
    X3D-S  & - & - & - & - & 3.4 & 1.96 & 72.9  \\ \hline
     \multirow{4}{*}{Manual}  & 2 & - & - & -  & 3.5 & 2.33 & 72.6 \textcolor{purple}{(\textbf{$-$0.3})} \\
     & - & 2 & - & - & 3.6 & 2.56  & 73.0 \textcolor{c_green}{(\textbf{$+$0.1})} \\
     & - & - & 2 & - & 3.7 &  2.39 & 72.8 \textcolor{purple}{(\textbf{$-$0.1})} \\
     & - & - & 2 &  3 & 5.4 & 2.92  &  73.0 \textcolor{c_green}{(\textbf{$+$0.1})} \\ \hline
    Automatic & \multicolumn{4}{c|}{Searched} & 4.1 & 2.44  &  \textbf{73.3} \textcolor{c_green}{(\textbf{$+$0.4})}  \\
\bottomrule
% \specialrule{.1em}{.05em}{.05em}

  \end{tabular}
}
\vspace{-3pt}
\caption{\textbf{Ablation in attention block insertion location}. The number $k$ under column S$n$ denotes $k$ attention blocks are uniformly placed in stage $n$. 
}
\label{tab:search_attention}
\vspace{-5pt}
\end{table}

To ablate the importance of attention block search, we conduct an ablation study based on the original X3D-S~\cite{x3d} backbone by 1) Manually insert attention block in each stage; 2) Automatically search the suitable position of attention block through probabilistic search algorithm~\cite{2019pnas}. We then compare them with the original baseline (X3D-S) on Kinetics-400 testbed. 

As shown in Table \ref{tab:search_attention}, the first row represents the X3D-S baseline, reaching 72.9\% top-1 accuracy with 1.96 GFLOPs cost. The second row includes four different architectures, where the attention blocks are inserted to different positions, ranging from the shallow layer (stage 1) to the deep layer (stage 4). These limited manual attempts bring minor improvement ($+$\textbf{0.1\%}) based on the X3D-S backbone and sometimes even hurt the performance ($-$\textbf{0.3\%}), motivating us to apply the automatic tools (\eg, NAS) to reap the performance benefits of various position choices. We finally adopted the probabilistic-based architecture search on discovering the suitable position of attention blocks, where a block-wise position search is conducted with the rest of the backbone being fixed. To this end, the searched architecture reaches 73.3\% top-1 accuracy, surpassing the original X3D-S baseline by a notable margin (\textbf{$+$0.4\%}) with a comparable FLOPs cost.

\subsubsection{Evaluation of Fairness-Aware Search}
\label{sec:exp_fairness_filter_number}
The default channel search simply split the super kernel into $N$ splits and sample the candidate by default order. As we discussed in Sec.~\ref{sec:fair_channel_selection}, this naive selecting strategy will make some parts of the super kernel to be over-sampled and updated unfairly. Thus the discovered model will easily collapse to the candidate which is updated more frequently. 

To better understand the effectiveness of the proposed fairness-aware sample strategy, we conduct experiments that only search for the output channel and expansion ratio by separately using these two sampling strategies, while other factors are fixed.
As shown in Figure \ref{fig:flops_curve}, the blue curve represents the FLOPs cost of discovered architectures during the search process by using the naive channel selection strategy, and the red curve represents the fairness-aware one. Given a target FLOPs, the naive channel selection strategy easily collapses to the smaller subnets, due to the smaller channel candidates are updated more frequently than others in each super kernel. In contrast, the fairness-aware strategy can discover a more suitable subnet that is closer to the target FLOPs cost. The collapsed discovered architecture, shows poor performance after evaluation, with a large margin ($-$\textbf{2.6\%}) behind the well-discovered fairness-based one. Details are shown in Table \ref{tab:cost}.


\begin{figure}[t!]
\vspace{-3pt}
    \centering
\includegraphics[width=\linewidth]{figs/cost_curve.pdf}   
\vspace{-8pt}
\caption{\textbf{FLOPs during searching.} For each epoch (x-axis), we derive the most probable architecture and measure its FLOPs (y-axis). The target FLOPs $T$ (Equation \ref{eq:cost}) is set to 2.0 GFLOPs.}
    \label{fig:flops_curve}
    % \vspace{-3pt}
\end{figure}


% The accuracy and FLOPs of the searched architectures are presented in Table \ref{tab:cost}. The architecture searched with the naive channel selection mechanism has much lower FLOPs than the target FLOPs, while the FLOPs of the architecture searched with fair channel selection is on par with the target FLOPs. Also, the architecture searched with our proposed achieves much better video accuracy than the naive channel selection method ($70.5\%$ vs $73.1\%$).
\begin{table}[t!]
\centering
\resizebox{\linewidth}{!}{
  \begin{tabular}{l|c|c|c}
  \toprule
  \multirow{2}{*}{Search Strategy} & Target & Discovered  & Accuracy (\%) \\ 
   & FLOPs (G) & FLOPs (G) & Top-1 \\\specialrule{.1em}{.1em}{.1em}
  Naive Channel Selection & \multirow{2}{*}{2.0} & 1.7\textcolor{purple}{($-$\textbf{0.3})} & 70.5 \textcolor{purple}{($-$\textbf{2.6})} \\
  Fair Channel Selection (\textbf{ours}) &  & \textbf{2.0} & \textbf{73.1}  \\
  \bottomrule
  \end{tabular}
}
  \caption{\textbf{Architecture search with different channel selection mechanisms.}}
\label{tab:cost}
% \vspace{-10pt}
\end{table}


==> WACV AutoX3D (camera ready)/tex/5_5_comparison_sota.tex <==
\subsection{Comparing \autoxthreed Models with Others}
\label{sec:comparison_sota}
In this section, we compare our searched \autoxthreed models with other SOTA models. 
\vspace{-1.em}
\subsubsection{Results on Kinetics}
\begin{table}[!t]
% \vspace{-0.8cm}
\centering
{\small
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{1mm}{
    \begin{tabular}{l|c|c|c|c|c}
    \toprule
    Model & Pretrain & Top-1 & Frames & GFLOPs$\times$Views & Param.\\
  \specialrule{.15em}{.1em}{.1em}      
    I3D \cite{carreira2017quo} & ImgNet & 71.1 & 64 & 108 $\times$ N/A & 12.0 \\
    2-Stream I3D \cite{carreira2017quo} & ImgNet  & 75.7 & 64 & 216 $\times$ N/A & 25.0 \\
    MF-Net \cite{chen2018multi} & ImgNet  & 72.8 & 16 & 11.1 $\times$ 50 & 8.0 \\
    TSM R50 \cite{tsm} & ImgNet  & 74.7 & 16 & 65.0 $\times$ 10 & 24.3 \\
    S3D-G \cite{xie2018rethinking} & - & 74.7& 64 & 71.0 $\times$ N/A & N/A \\
    
    % \midrule
     
    2-Stream I3D \cite{carreira2017quo} & - & 71.6 & 64 & 216 $\times$ N/A & 25.0 \\
    R(2+1)D \cite{tran2018closer} & - & 72.0 & 32 & 152 $\times$ 115 & 63.6 \\
    2-Stream R(2+1)D \cite{tran2018closer} & - & 73.9 & 32 & 304 $\times$ 115 & 127 \\
    ip-CSN-50 \cite{csn} & - & 70.8 & 8 & 11.9 $\times$ 30 & 14.3 \\
    ip-CSN-101 \cite{csn} & - & 71.8 & 8 & 15.9 $\times$ 30 & 24.5 \\
    % SlowFast 4×16, R50 \cite{slowfast} & - & 75.6 & 92.1 & - & 36.1 $\times$ 30 & 34.4M\\
    % SlowFast 8×8, R101 \cite{slowfast} & - & 77.9 & 93.2 & 84.2 & 106 $\times$ 30 & 53.7M\\
    % SlowFast 8×8, R101+NL \cite{feichtenhofer2019slowfast} & - & 78.7 & 93.5 & 84.9 & 116 $\times$ 30 & 59.9M &\\
    % SlowFast 16×8, R101+NL \cite{feichtenhofer2019slowfast} & - & 79.8 & 93.9 & 85.7 & 234 $\times$ 30 & 59.9M &\\ 
    % X3D-L \cite{x3d} & - & 77.5 & 92.9 & 83.8 & 24.8 $\times$ 30 & 6.1M &\\
    % X3D-XL \cite{x3d} & - & 79.1 & 93.9 & 85.3 & 48.4 $\times$ 30 & 11.0M &\\
    % X3D-XXL \cite{x3d} & - & 80.4 & 94.6 & 86.7 & 194.1 $\times$ 30 & 20.3M &\\
    \midrule
    TSM Mb-V2 \cite{tsm} & ImgNet & 69.5& 16 & 6.0 $\times$ N/A & 3.9 \\
    % MobileNetV2-3D$_{8F}$  & - & - & - & 8 & 3.25 $\times$ 30 & 4.4M \\
    VoV3D-M~\cite{lee2020diverse} & - & 73.9 & 16 & 4.4 $\times$ 30 & 3.8 \\
    X3D-S~\cite{x3d} & - & 73.3 & 13 & 2.7 $\times$ 30 & 3.8 \\
    
    % \textbf{AutoX3D-S} & - & \textbf{73.2} & \textbf{91.1} & 13 & 2.7 $\times$ 30 & 4.0 \\
    % AutoX3D-S w/o attn. & - & 74.1 & 13 & 2.7 $\times$ 30 & 3.7 \\
    \textbf{AutoX3D-S} & - & \textbf{74.7} & 13 & 2.9 $\times$ 30 & 3.5 \\
    
     
    \midrule
    MobileNetV2-3D (impl.)  & - & 71.2 & 16 & 6.5 $\times$ 30 & 4.4 \\
    SlowFast 4×16, R50 \cite{slowfast} & - & 75.6 & 16 & 36.1 $\times$ 30 & 34.4 \\
    % EfficientNetB3-3D~\cite{x3d}  & - & 72.4 & 89.6 & 16 & 6.91 $\times$ 10 & 8.2 \\
    VoV3D-L~\cite{lee2020diverse} & - & 76.3 & 16 & 9.3 $\times$ 30 & 6.2 \\
    X3D-M~\cite{x3d} & - & 76.0 & 16 & 6.2 $\times$ 30 & 3.8 \\
    % \textbf{AutoX3D-M} & - & \textbf{} & \textbf{} & 16 &  $\times$ 30 & 4.0 \\
    % AutoX3D-M w/o attn. & - & 76.3 & 16 & 6.2 $\times$ 30 & 3.7 \\
    \textbf{AutoX3D-M} & - & \textbf{76.7}& 16 & 6.8 $\times$ 30 & 3.5 \\
    % \textbf{AutoX3D} & - & \textbf{73.2} & - & 16 & 4.97 $\times$ 30 & 6.6 \\ 
    \midrule
    % EfficientNetB4-3D~\cite{x3d}  & - & 74.5 & 90.6 & 16 & 23.8 $\times$ 10 & 12.2M \\
    SlowFast 8×8, R101 \cite{slowfast} & - & 77.9 & 8 & 106 $\times$ 30 & 53.7 \\ 
    X3D-L & - & 77.5 & 16 & 24.8 $\times$ 30 & 6.1 \\
    X3D-XL & - & 79.1 & 16 & 48.4 $\times$ 30 & 11.1 \\
    \textbf{AutoX3D-L} & - & \textbf{78.8} & 16 & \textbf{27.8} $\times$ 30 & 6.2 \\
    \bottomrule
    \end{tabular}
    }
  }
}
\vspace{-0.5em}
\caption{\textbf{Comparison with the state-of-the-art methods on Kinetics-400 dataset}. We use (GFLOPs $\times$ views) to represents inference cost $\times$ number of views).}
\label{tab:kinetics_sota}
\vspace{-10pt}
\end{table}

We mainly follow the comparison convention of X3D \cite{x3d} on popular large-scale benchmarks, and compare the performance of our AutoX3D with current state-of-the-art efficient architectures. 
% We firstly conduct experiments on Kinetics-400 dataset  \cite{carreira2017quo}, details are shown in Table. \ref{table:Kinetics}. 
The Top-1 accuracy as well as the FLOPS cost are reported on Kinetics-400 dataset. We divide the models into four categories according to their FLOPs cost, shown in Table \ref{tab:kinetics_sota}. The first group includes previous high-performance yet inefficient methods. Those methods either cost more FLOPs and parameters compared to ours, or get worse performance. In the second group, the proposed AutoX3D-S architecture achieves 74.7\% accuracy, better than TSM with mobilenet backbone ($+$\textbf{5.2\%}), VoV3D-M ($+$\textbf{0.8}\%), and X3D-S ($+$\textbf{1.4}\%). Regarding FLOPs, AutoX3D-S costs $\times$\textbf{2} smaller FLOPs than TSM with mobilnet backbone, $\times$\textbf{1.5} smaller FLOPs than VoV3D-M, and comparable FLOPs compared to X3D-S. In the third group,
we evaluate a larger architecture, named AutoX3D-M, which is derived from AutoX3D-S by increase the input frame number to 16 and input video spatial resolution to 256. 
It achieves 76.7\% accuracy, largely outperforms our implemented MobileNetV2-3D ($+$\textbf{5.5\%}) and SlowFast 4x16 ($+$\textbf{1.1\%}), respectively. Compared to X3D-M, AutoX3D-M obtains $+$\textbf{0.7\%} higher accuracy with similar FLOPS cost. In the fourth group, we present our biggest architecture AutoX3D-L by scaling the network depth of AutoX3D-M to $\times$2 deeper and increasing the input video spatial resolution to 356. AutoX3D-L surpasses X3D-L by $\textbf{1.3\%}$ accuracy with similar FLOPs cost, and reaches comparable performance compared to X3D-XL with much smaller ($\times$\textbf{1.74}) FLOPs cost.
% while the FLOPs cost is on par with X3D-L. 
% In the fourth group, to evaluate the scalability of searched architectures, we scale up the AutoX3D-k2 by increasing its depth to 1.46$\times$ layer. 
\vspace{-1.em}
\subsubsection{Results on Something-Something-V2}
\begin{table}[t!]
\centering
{\small
\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{1mm}{
    \begin{tabular}{l|c|c|c|c|c}
    \toprule
    Model & Pretrain &  Top-1  & Frames & GFLOPs & Param. (M)\\
  \specialrule{.15em}{.1em}{.1em}   
    TSM$_{8F}$ \cite{tsm} & \multirow{11}{*}{ \rotatebox[origin=c]{90}{ImageNet}   } & 59.1 & 8 & 32.9 & 23.9 \\
    TSM$_{16F}$ \cite{tsm} &  & 63.4 & 16 & 65.8 & 23.9 \\
    STM$_{8F}$ \cite{stm} &  & 62.3  & 8 & 33.3 & 24.0 \\
    STM$_{16F}$ \cite{stm} &  & 64.2 & 16 & 66.5 & 24.0 \\
    GST${_8F}$ \cite{GST}  &  & 61.6  & 8 & 35.4 & - \\
    GST${_16F}$ \cite{GST} &   & 62.6  & 16 & 35.4 & - \\
    I3D + STIN + OIE \cite{STIN} &  & 60.2  & - & - & - \\
    Dynamic Inference \cite{wu2020dynamic} &  & 58.2  & - & 35.4 & - \\
    % TANet \cite{TANet} &  & 64.6 & 16 & - &  25.6 \\
    SmallBigNet$_{8F}$ \cite{SmallBigNet} &  & 61.6 & 8 & 52 & - \\
    SmallBigNet$_{16F}$ \cite{SmallBigNet} &  & 63.8  & 16 & 105 & - \\
    \hline
    X3D-S & \multirow{4}{*}{-} & 61.3 & 13 & 2.0 & 3.8 \\
    X3D-M &  & 62.7 & 16 & 4.7 & 3.8 \\
    % \hline
    % X3D-S~\cite{x3d} & \multirow{2}{*}{Kinetics400}  & 58.3 & - & 13 & 1.96 & 4.4 \\
    % AutoX3D-S & \multirow{2}{*}{4}  & \textbf{62.1} &  13 & 2.04 & 4.1 \\
    \textbf{AutoX3D-S} &  & 62.1 & 13 & \textbf{2.2} & 3.5 \\
    \textbf{AutoX3D-M} &  & \textbf{63.4} & 16 & \textbf{5.3} & 3.5 \\
    \bottomrule
    \end{tabular}
    }
  }
}
% \vspace{-0.5em}
\caption{\textbf{Comparison with the state-of-the-art methods on Something-Something-V2 dataset}. }
% \vspace{-5pt}
% \vspace{-10pt}
% By default, we adopt uniform-sampling, which firstly divides the video sequence into $n$ uniform segments and then picks a random frame from each segment as the input frame.}
% \zhicheng{explain what is uniform sampling}.
\label{tab:sthsthv2_sota}
\end{table}
In addition, we directly transfer the discovered architectures on Something-something v2 dataset. We include current state-of-the-art methods in Table \ref{tab:sthsthv2_sota}, where AutoX3D model family achieves competitive performance \textbf{without} the necessity of pre-training. For example,
AutoX3D-S achieves similar accuracy (62.1\% vs 62.3\%) with STM$_{8F}$ while the FLOPs cost is $\times$\textbf{15} smaller. The Top-1 accuracy of AutoX3D-M is on par with SmallBigNet$_{16F}$ (63.4\% vs 63.8\%), while the FLOPs cost is \textbf{$\times$20} fewer.
%AutoX3D-S outperforms Non-local I3D (1.3\%) and TSM R50 (0.1\%) with much fewer FLOPs. Moreover, AutoX3D-S is 0.7\% higher than X3D-M with nearly the same FLOPs. These impressive results verify both the high performance and transfer-ability of our NAS framework.



==> WACV AutoX3D (camera ready)/tex/5_6_understand_autox3d.tex <==
\subsection{Understanding \autoxthreed Architectures}
\label{sec:understand_autox3d}
\begin{figure}[t]
    \centering
\includegraphics[width=\linewidth]{figs/arch.pdf}  
\caption{Visualization of the searched architecture. The number in each block represents the base channel of 3D MBConv block. The wider width of the block denotes the higher expansion ratio.}
    \label{fig:vis_arch}
    % \vspace{-5pt}
\end{figure}
% Our searched \autoxthreed architectures are visualized in Fig TBD.
% \textcolor{red}{We study the architecture pattern of the discovered AutoX3D models in Figure~\ref{fig:vis_arch}. For backbone, we can observe that the spatial kernel size of 5 and temporal kernel size of 1 are widely used in both streams, along the network, which is quite different from the design in current hand-crafted models. Surprisingly, we notice that the attention blocks only appear on the sparse stream, indicating they are less effective on dense stream. Unlike manual designed architectures which often favors the uniform choices of search variables, the searched network becomes quite nonuniform.}
 Our searched \autoxthreed architectures are visualized in Figure~\ref{fig:vis_arch}. Regarding to the design of the backbone network, we find that $3 \times 3^2 $ convolution is widely adopted, while temporal kernel size 5 is hardly used. We also observe that $5 \times 5^2$ convolution is never used in our network, due to its high complexity.
 Interestingly, We also find that the expansion ratio is often higher at the first block of each stage (except stage 1).
 

==> WACV AutoX3D (camera ready)/tex/6_conclusion.tex <==
\section{Conclusions and Future Work}
In this paper, we introduce a family of efficient AutoX3D models, by directly searching without using any architecture surrogate nor hand-crafted image architecture. The proposed efficient architectures are discovered through a finer-grained search space, where block type, filter number, expansion ratio and attention block are jointly searched. In addition, a fairness-aware search strategy is adopted to avoid collapse issue. Our best architecture achieves state-of-the-art performance both on Kinetics-400 dataset and Something-something-V2 dataset, \eg, $+$\textbf{1.3}\% accuracy compared to X3D-L, and $\times$\textbf{1.74} lower computational cost compared to X3D-XL, on Kinetics-400 validation set.


% In this paper, we present AutoX3D, adopting a powerful tool of neural architecture search (NAS) to extend X3D \cite{x3d} and greatly reduce the computation of original grid-search. Specifically, we introduce a gigantic fine-grained search space that completely allowing block types, channel numbers, and expansion ratios searchable. 
% Different from conventional differentiable search, our search space is depth-aware to reflect the progressively varying temporal-spatial feature pattern along with the layer depth. 
% Based on this, we analyze the discovered architectures and conclude the insight of temporal modeling principle under the framework of MobileNet structure. While the Top-heavy modeling strategy is still proved its effectiveness under MobileNet backbone, a surprising finding is that separately convolving spatial and temporal features (S3D) do not show their superiority as how it performs in ResNet or Inception based model. As AutoX3D mainly explores efficient architectures, we will extend our work to the large-scale model in future work.

==> WACV AutoX3D (camera ready)/tex/backup_fairness_filter_number_selection.tex <==


\subsection{Fairness-Aware Search of Filter Number}
\label{sec:exp_fairness_filter_number}

In Section~\ref{sec:fair_channel_selection}, we proposed fairness-aware search of filter number to ensure that the weights, which are shared by the choices of filter number, for each convolutional filter are updated with a fair chance at the beginning stage of the search. To study the importance of such fairness, we search for the architecture with the vanilla channel masking, where weights of the convolutional filters in the lower rank are more frequently updated. 
%We firstly analyze the supernet accuracy curve in the search stage, as shown in \textcolor{red}{xxx}. Thanks to the help of fair channel selection strategy, each activated sub-network is updated with the same frequency and can be fairly evaluated thus the accuracy curve is more stable. The network FLOPs of the vanilla channel masking quickly collapse to a small value, which we hypothesis this is due to the unbalanced on channels.
We analyze the searched architecture FLOPs in Fig. \ref{fig:flops_curve}. We conduct two searching experiments that one with the naive channel selection mechanism and the other one with our proposed fair channel selection. Other hyper-parameters are kept identical. We only search for the output channel and expansion ratio in those experiments. Thanks to the help of fair channel selection mechanism, each activated sub-network is updated with similar frequency and can be fairly evaluated, thus prevent the tendency of collapsing to select the well-updated small channel in the naive channel selection mechanism. We can observe the curve of FLOPs cost term of naive channel selection mechanism quickly collapse to zero, while ours is approaching to the target FLOPs steadily. 
%We found that the FLOPs cost term of the one with the naive channel selection mechanism collapse more quickly than the one with our fiar channel selection mechanism.
% We find the performance of searched results will generally decrease around $0.5\%$. %, details will be shown in the supplementary.
\begin{figure}[t!]
    \centering
\includegraphics[width=\linewidth]{figs/flops_curve.png}   
\caption{\textbf{FLOPs during searching.} For each epoch (x-axis), we derive the most probable architecture and measure its FLOPs (y-axis).}
    \label{fig:flops_curve}
\end{figure}

The accuracy and FLOPs of the searched architectures are presented in Tab. \ref{tab:cost}. The architecture searched with the naive channel selection mechanism has much lower FLOPs than the target FLOPs, while the FLOPs of the architecture searched with fair channel selection is on par with the target FLOPs. Also, the architecture searched with our proposed achieves much better video accuracy than the naive channel selection method ($70.5\%$ vs $73.1\%$).
\begin{table}[t!]
\centering
\resizebox{\linewidth}{!}{
  \begin{tabular}{l|c|c|c}
  \toprule
  \multirow{2}{*}{Search Strategy} & Target & Discovered  & Accuracy (\%) \\ 
   & FLOPs (G) & FLOPs (G) & Top-1 \\\specialrule{.1em}{.1em}{.1em}
  Naive Channel Selection & \multirow{2}{*}{2.0} & 1.7\textcolor{purple}{($-$\textbf{0.3})} & 70.5 \textcolor{purple}{($-$\textbf{2.6})} \\
  Fair Channel Selection (\textbf{ours}) &  & \textbf{2.0} & \textbf{73.1}  \\
  \bottomrule
  \end{tabular}
}
  \caption{\textbf{Architecture search with different channel selection mechanism.}}
\label{tab:cost}
\end{table}


==> WACV AutoX3D (camera ready)/tex/backup_search_glore.tex <==


\subsection{Searching for Attention Block}
% The placement location of attention blocks usually plays a significant role in the accuracy improvement of network. 
\begin{table}[t!]
% \vspace{-0.6cm}
\centering
% \small
% \tiny
% \scriptsize
\resizebox{\linewidth}{!}{

  \begin{tabular}{c|cccc|c|c|c}
  \toprule
     \multirow{2}{*}{Model} &  \multicolumn{4}{c}{Attention location}  & Params & FLOPS & \multicolumn{1}{c}{Accuracy ($\%$)} \\
    & S1 & S2 & S3 & S4 & (M) & (G) & Top-1 \\
    \specialrule{.1em}{.1em}{.1em}
    X3D-S  & - & - & - & - & 3.4 & 1.96 & 72.9  \\ \hline
     \multirow{4}{*}{Manual}  & 2 & - & - & -  &  &  & 72.6 \textcolor{purple}{(\textbf{$-$0.3})} \\
     & - & 2 & - & - &  &   & 73.0 \textcolor{c_green}{(\textbf{$+$0.1})} \\
     & - & - & 2 & - &  &   & 72.8 \textcolor{purple}{(\textbf{$-$0.1})} \\
     & - & - & 2 &  3 &  &   &  73.0 \textcolor{c_green}{(\textbf{$+$0.1})} \\ \hline
    Automatic & \multicolumn{4}{c}{Searched}   &  &   &  \textbf{73.3} \textcolor{c_green}{(\textbf{$+$0.4})}  \\
\bottomrule
% \specialrule{.1em}{.05em}{.05em}

  \end{tabular}
}
\caption{\textbf{Ablation in attention block insertion location}. The number $k$ under column S$n$ denotes $k$ attention blocks are uniformly placed in stage $n$. 
%\textit{VG} and \textit{DG} denotes vanilla GloRe block and Dual-GCN GloRe block, respectively. 
}
\label{tab:search_attention}
\end{table}



In the original GloRe paper\cite{glore}, 2 and 3 GloRe blocks are placed in stage 3 and stage 4 of the network respectively. We argue that such placement arrangement might not be the optimal setting. In this section, we adopt X3D-S as the baseline network, and only search for the placement locations of attention blocks. We also manually insert attention blocks into the network to create some manual-designed baselines. The configuration and results are shown in Tab. \ref{tab:search_attention}. Surprisingly, we observe that models with different attention locations perform quite differently. Improper insertion locations might even hurt the network performance. For example, inserting two GloRe in stage 1 brings inferior performance compared to X3D-S (\textcolor{red}{xx} vs $72.9\%$). We also find that the searched one brings better performance (\textcolor{red}{xx} vs $72.9\%$). Those experiments firmly demonstrate that the placement location of attention blocks is worth to be searched.



==> WACV AutoX3D (camera ready)/tex/broader_impact.tex <==

\section*{Broader Impact}
This work will inspire the human to better adopt artificial intelligence (AI) as a useful tool to improve our life. Since there is an increasing number of people uploading and watching videos in the Internet, it is an important topic about how we improve the user experiences in video websites. As a typical example, there are more than $10^5$ hours videos uploaded to YouTube in a day, and those need to be efficiently and effectively processed for recommendation system. The computer vision community has been working for decades to study diverse video analysis problem such as action recognition/understanding. The majority of latest video recognition models are computationally heavy, often using deeper/wider networks and high space-time resolution. Those expensive models turn impractical for nearly real-time or low-latency applications in mobile vision. To this end, successful design knowledge and building blocks for efficient image recognition models have been transplanted into video models too, including R(2+1)D \cite{tran2018closer}, TSM\cite{lin2019tsm}, MixTConv\cite{shan2020mixtconv}, and Video Shuffle Network\cite{ma2019learning}.

In this work, we propose an automatics algorithm to build the ultra-efficient video models. We take steps further towards the direction of extremely light-weight and efficient video recognition models. The goal is fundamentally challenging as it needs to combine the following two: (1) exploring the temporal-spatial feature patterns and their fusion across the network layers; and (2) integrating the variety of efficient network modules and other design options into the network. 
% The complicacy is further amplified by the model training workload on large-scale video recognition datasets. Such a daunting goal makes it no longer feasible to proceed with manual trial-and-errors.

Besides the benefits of video understanding itself, another goal of this work is to save energy and reduce carbon dioxide ($CO^2$) emissions which helps prevent greenhouse effect. As previous works \cite{feichtenhofer2020x3d, xie2018rethinking} spend much time on designing effective hand-crafted model, or use a computationally expensive way to search the diverse architectures (E.g. RL \cite{ryoo2019assemblenet}, Evolution \cite{piergiovanni2019tiny}), the design and search cost is extremely large. We firstly introduce a differentiable search algorithm to enables the block-type, channel numbers, expansion ratios, and input frames to be completely search. The search cost is largely reduced thanks to the weight sharing strategy and the searched architecture is both efficient and effective.

Despite the advantages of Auto-X3D, one potential concern is the user privacy security. Since deep learning method typically required gigantic data for training, the ill-use of user data may cause privacy violation. We would encourage the company to properly adopt automatic video analysis tool on their application and take care of the user privacy.

==> WACV AutoX3D (camera ready)/tex/ignore_5_3_search_backbone.tex <==
\subsection{Searching For Backbone w/o Attention Blocks}
\label{sec:search_backbone}

Our design space allows variable choices of block micro-architecture, filter number, expansion rate and attention blocks at different depth of the model. In contrast, the X3D~\cite{x3d} models not only use uniform micro-architecture, heuristic choices of filter number and constant expansion rate, but also lack the use of attention blocks as in our design space. In the first study where our focus is to fairly compare our searched models with the X3D models, we adopt a reduced design space where attention blocks are not used. Equivalently, that means in the macro-architecture of our space (Table~\ref{tab:macro-arch}), we do not add any attention block after each MBConv-3D block group.

We call our model searched in this reduced space as \autoxthreedS. During architecture evaluation, when we use an input size $T\times S^2 = 16\times224^2$, which is larger than input size $13\times160^2$ during architecture search, but keep the architecture unchanged, the model is called s as \autoxthreedM, following the convention in X3D. The results are shown in Table~\ref{tab:search_backbone}. By searching the block-type, filter number, and expansion ratio, \autoxthreedS achieves \textcolor{red}{xxx} accuracy and outperforms the hand-crafted X3D-S models by \textcolor{red}{xxx}. Meanwhile, \autoxthreedM is \textcolor{red}{xxx} higher than X3D-M with nearly the same FLOPs cost.

% zhicheng: add a dummy box to take the space which is expected to include discussions on the results in table tab:search_backbone
% \begin{solutionorbox}
% \vspace{4cm}
% \end{solutionorbox}

\begin{table}[t]
% \vspace{-0.6cm}
\centering
% \small
% \tiny
% \scriptsize
\resizebox{0.4\textwidth}{!}{

  \begin{tabular}{c|c|c|cc}
       \multirow{2}{*}{Model} & Params & FLOPS & \multicolumn{2}{c}{Accuracy ($\%$)} \\
       &  (M) & (G) & Top-1 & Top-5 \\
    \specialrule{.15em}{.1em}{.1em}
    
    X3D-S &  3.76 & 1.96  & 72.1* & \\
    \autoxthreedS   & 3.82* & 1.95*  & 72.9*  & \\ \hline
    X3D-M &  3.76 & 4.73  & 74.5* &  \\
    \autoxthreedM   & 3.82* & 4.76*  & 75.3*  &  \\

% \specialrule{.1em}{.05em}{.05em}

  \end{tabular}
}
\caption{\textbf{Comparisons to X3D models}. We evaluate them on Kinetics, and results of 10-Center testing are reported. }
\label{tab:search_backbone}
\end{table}

==> WACV AutoX3D (camera ready)/tex/ignore_5_4_search_in_full_space.tex <==
\subsection{Searching in the Full \autoxthreed Space}
\label{sec:exp_search_attention_blocks}

 Attention mechanism \cite{glore,nonlocal_block} has been demonstrated for its strong performance on both image and video benchmark. However, the poor efficiency of non-local block raises a major concern when applying on efficient architecture design. We evaluate the performance of both non-local unit and global reasoning unit on the ultra-efficient backbone X3D. As shown in Table. \ref{tab:search_in_full_space}, inserting different global reasnoning unit on different postion (from shadow to deep) mostly achieves a impressive improvement with few FLOPs cost, while non-local block costs much larger FLOPs in the early stage. This demonstrates the effectiveness and efficiency of global reasoning unit \cite{glore} and further motivate us to apply automatic search in terms of the block type and inserting position for global reasnong unit. Therefore, we search architectures in the full \autoxthreed space, where we jointly search the choices of block micro-architecture, filter number, expansion rate and attention block type for individual MBConv-3D block groups. The searched models from the full space are called as \autoxthreedSplus model. 

% Compared with the searched \autoxthreedS models in Section~\ref{sec:search_backbone}, attention blocks of the searched type are added to each block group in \autoxthreedSplus model. To highlight the importance of searching attention block types, we also build a strong baseline by manually inserting GloRe blocks to \autoxthreedS models. The results are shown in Table~\ref{tab:search_in_full_space}.

% \zhicheng{add discussions on the results in Table~\ref{tab:search_in_full_space}}.



% zhicheng: add a dummy box to take the space which is expected to include discussions on the results of searching attention blocks


==> WACV AutoX3D (camera ready)/tex/old_5_3_external_exp.tex <==
\subsection{Comparison with State-of-the-Art Models}


\begin{table*}[!t]
% \vspace{-0.8cm}
\centering
{\small
\resizebox{0.9\linewidth}{!}{
\setlength{\tabcolsep}{0.9mm}{
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
    % \toprule
    Model & Pretrain & Top-1 ($\%$) & Top-5 ($\%$) & \# Frames & GFLOPs$\times$ views & #Param (M)\\
  \specialrule{.15em}{.1em}{.1em}      
    I3D \cite{carreira2017quo} & ImgNet & 71.1 & 90.3 & 64 & 108 $\times$ N/A & 12.0 \\
    Two-Stream I3D \cite{carreira2017quo} & ImgNet  & 75.7 &  & 64 & 216 $\times$ N/A & 25.0 \\
    MF-Net \cite{chen2018multi} & ImgNet  & 72.8 & 90.4 & 16 & 11.1 $\times$ 50 & 8.0 \\
    TSM R50 \cite{lin2019tsm} & ImgNet  & 74.7 & N/A & 16 & 65 $\times$ 10 & 24.3 \\
    S3D-G \cite{xie2018rethinking} & - & 74.7 & N/A & 64 & 71.0 $\times$ N/A & N/A \\
    
    % \midrule
    
    Two-Stream I3D \cite{carreira2017quo} & - & 71.6 & 90.0 & 64 & 216 $\times$ N/A & 25.0 \\
    R(2+1)D \cite{tran2018closer} & - & 72.0 & 90.0 & 32 & 152 $\times$ 115 & 63.6 \\
    Two-Stream R(2+1)D \cite{tran2018closer} & - & 73.9 & 90.9 & 32 & 304 $\times$ 115 & 127 \\
    % ip-CSN-50 \cite{tran2019video} & - & 70.8 & - & 8 & 11.9 $\times$ 30 & 14.3M \\
    % ip-CSN-101 \cite{tran2019video} & - & 71.8 & - & 8 & 15.9 $\times$ 30 & 24.5M \\
    % SlowFast 4×16, R50 \cite{feichtenhofer2019slowfast} & - & 75.6 & 92.1 & - & 36.1 $\times$ 30 & 34.4M &\\
    % SlowFast 8×8, R101 \cite{feichtenhofer2019slowfast} & - & 77.9 & 93.2 & 84.2 & 106 $\times$ 30 & 53.7M &\\
    % SlowFast 8×8, R101+NL \cite{feichtenhofer2019slowfast} & - & 78.7 & 93.5 & 84.9 & 116 $\times$ 30 & 59.9M &\\
    % SlowFast 16×8, R101+NL \cite{feichtenhofer2019slowfast} & - & 79.8 & 93.9 & 85.7 & 234 $\times$ 30 & 59.9M &\\
    % X3D-L \cite{feichtenhofer2020x3d} & - & 77.5 & 92.9 & 83.8 & 24.8 $\times$ 30 & 6.1M &\\
    % X3D-XL \cite{feichtenhofer2020x3d} & - & 79.1 & 93.9 & 85.3 & 48.4 $\times$ 30 & 11.0M &\\
    % X3D-XXL \cite{feichtenhofer2020x3d} & - & 80.4 & 94.6 & 86.7 & 194.1 $\times$ 30 & 20.3M &\\
    \midrule
    TSM Mb-V2 \cite{lin2019tsm} & ImgNet & 69.5 & - & 16 & 6.00 $\times$ N/A & 3.9 \\
    % MobileNetV2-3D$_{8F}$  & - & - & - & 8 & 3.25 $\times$ 30 & 4.4M \\
    X3D-M$_{8F}$ \cite{feichtenhofer2020x3d} (our impl.) \cite{feichtenhofer2020x3d} & - & 69.3 & 88.6 & 8 & 2.47 $\times$ 30 & 4.4 \\
    \textbf{Auto-X3D-k1} & - & \textbf{70.7} & \textbf{89.4} & 8 & 2.50 $\times$ 30 & 6.0 \\
    \midrule
    MobileNetV2-3D (our impl.)  & - & 71.2 & 90.1 & 16 & 6.50 $\times$ 30 & 4.4 \\
    EfficientNetB3-3D from \cite{feichtenhofer2020x3d}  & - & 72.4 & 89.6 & 16 & 6.91 $\times$ 30 & 8.2 \\
    X3D-M$_{16F}$ \cite{feichtenhofer2020x3d} (our impl.\footnotemark) & - & 72.5 & 90.8 & 16 & 4.92 $\times$ 30 & 4.4 \\
    \textbf{Auto-X3D-k2} & - & \textbf{73.7} & \textbf{91.7} & 16 & 4.97 $\times$ 30 & 6.6 \\ 
    % \midrule
    % EfficientNetB4-3D from \cite{feichtenhofer2020x3d}  & - & 74.5 & 90.6 & 16 & 23.8 $\times$ 30 & 12.2M \\
    % \textbf{Auto-X3D-k3} & - & - &  & 16 & & \\ 
    \bottomrule
    \end{tabular}
    }
  }
}
\caption{\textbf{Comparisons to the state-of-the-art on Kinetics-400 dataset}. We use (GFLOPs $\times$ views) to represents inference cost $\times$ number of views). For evaluation, we uniformly sample 10 clips, and take 3 spatial croppings (i.e. Left, Center, and Right) per clip, and average the 30-view predictions.}
\label{table:Kinetics}
\end{table*}


\begin{table*}[t!]
\centering

\centering
{\small
\resizebox{0.95\linewidth}{!}{
\setlength{\tabcolsep}{0.9mm}{
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
    % \toprule
    Model & Backbone & Pretrain &  Top-1 ($\%$) & Top-5 ($\%$) & \# Frames & GFLOPs & #Param (M)\\
  \specialrule{.15em}{.1em}{.1em}      
    TSN \cite{zhou2018temporal}  & BNInception & ImgNet & 19.5 & - & 8 & 16 & 10.7 \\
    TSN from \cite{lin2019tsm}  & ResNet-50 & ImgNet & 19.7 & 46.6 & 8 & 33 & 10.7 \\
    TRN-Multiscale \cite{zhou2018temporal} & BNInception & ImgNet & 34.4 & - & 8 & 16 & 18.3 \\
    TRN-Multiscale from \cite{lin2019tsm} & ResNet-50 & ImgNet & 38.9 & 68.1 & 8 & 16 & 31.8 \\
    TSM \cite{lin2019tsm} & ResNet-50 & ImgNet & 45.6 & 74.2 & 16 & 33 & 24.3 \\
    ECO_{8F} \cite{zolfaghari2018eco} & BNInception+R3D-18 & - & 39.6 & - & 8 & 32 & 47.5 \\
    ECO_{16F} \cite{zolfaghari2018eco} & BNInception+R3D-18 & - & 41.4 & - & 16 & 32 & 47.5 \\
    % I2D \cite{xie2018rethinking} & Inception & - & 34.4 & 69.0 & 64 & & \\
    % I3D \cite{xie2018rethinking} & Inception & - & 45.8 & 76.5 & 64 & 108 & 12.06M\\
    I3D from \cite{wang2018videos} & R3D-50 & - & 41.6 & - & 32 & 153 & 28.0 \\
    % S3D \cite{xie2018rethinking} & Inception & - & 47.3 & 78.1 & 64 & 66 & 8.77M\\
    % S3D-G\cite{xie2018rethinking} & Inception & - & 48.2 & 78.7 & 64 & 71.38 & \\
    Non-local I3D from \cite{wang2018videos} & R3D-50 & - & 44.4 & 76.0 & 32 & 168 & 35.3 \\
    X3D-M$_{16F}$ \cite{feichtenhofer2020x3d} (our impl.) & MobileNet & - & 45.0 & 76.1 & 16 & 4.9 & 4.4 \\
    \textbf{Auto-X3D-k3} & MobileNet & - & \textbf{45.7} & \textbf{76.1} & 16 & 4.9 & 6.1 \\
    \bottomrule
    \end{tabular}
    }
  }
}
\caption{\textbf{Comparisons to the state-of-the-art on Something-Something-V1}. By default, we adopt uniform-sampling, which firstly divides the video sequence into $n$ uniform segments and then picks a random frame from each segment as the input frame. }
% \zhicheng{explain what is uniform sampling}.
\label{table:sthsthv1}
\end{table*}

% \footnotetext[2]{The original TVN paper \cite{piergiovanni2019tiny} reported no results on those benchmarks. Despite our best efforts to reproduce their methods and implement on the two datasets, their evolutionary algorithms were found to be ineffective in our experiments, whose results appear to be not reasonably competitive in Tables 2 and 3. We would be keen to include TVN into our comparison once their open-source implementations become available.}



We mainly follow the comparison convention of X3D \cite{feichtenhofer2020x3d} on popular large-scale benchmarks, and compare the performance of our Auto-X3D with current state-of-the-art efficient architectures\footnotemark . 
% We firstly conduct experiments on Kinetics-400 dataset  \cite{carreira2017quo}, details are shown in Table. \ref{table:Kinetics}. 
Top-1 accuracy as well as FLOPS are reported on Kinetics-400 dataset. We divide the models into three categories according to their FLOPs, details are shown in Table \ref{table:Kinetics}. The first group includes previous high-performance yet inefficient methods. Those methods either cost more FLOPs and parameters compared to ours, or get worse performance. In the second group, Auto-X3D-K1 achieves 70.7\% accuracy, better than TSM with mobilenet backbone (+1.2\%) and X3D-M$_{8F}$ (+1.4\%). Regarding FLOPs, Auto-X3D-k1 is 2.4$\times$ smaller than TSM with mobilnet backbone and costs comparable FLOPs compared to X3D-M$_{8F}$. In the third group, we evaluate a larger searched results named Auto-X3D-k2, it achieves 73.6\% accuracy and largely outperforms MobileNetV2-3D$_{16F}$ (2.5\%) and EfficienNet-B3-3D (1.3 \%), with 1.30$\times$ and 1.39 $\times$ smaller FLOPs respectively. Compared to X3D-M$_{16F}$, Auto-X3D-k2 reaches 1.2\% higher accuracy with similar FLOPS cost. 
% In the fourth group, to evaluate the scalability of searched architectures, we scale up the Auto-X3D-k2 by increasing its depth to 1.46$\times$ layer. 

In addition, We further apply the searched architecture on Kinetics to train on Something-something v1 dataset in order to demonstrate the generalization of discovered architectures. We include current state-of-the-art methods in Table \ref{table:sthsthv1}. Auto-X3D-k3 outperforms Non-local I3D (1,3\%) and TSM R50 (0.1\%) with much less FLOPs. Moreover, Auto-X3D-k3 is 0.7\% higher than X3D-M$_{16F}$ with nearly same FLOPs. These impressive results verify both the high performance and transferability of our NAS framework.













==> WACV AutoX3D (camera ready)/tex/old_5_4_ablation_study.tex <==
\subsection{Ablation Studies}
\begin{figure*}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}} 
 \includegraphics[width=\linewidth]{figure/Visualize.pdf}
\end{center}
% \vspace{-1em}
   \caption{\textbf{Discovered architectures}. The length of each block represents the expansion ratio and the filter number is marked inside the block. We find that the bottom-layers mostly choose spatial operator while the top-layers mostly choose temporal operators. This finding is consistent with previous conclusion on inception-based architectures \cite{xie2018rethinking}.}
%   \zhicheng{The caption is weak, and the figure is too simple now. Can you encode the width/expansion rate in the architecture as well? How does the searched arch resonate the top-heavy/bottom-heavy findings in hand-crafted models? Can you discuss a bit in caption?} 
\label{fig:visual}
\end{figure*}

\paragraph{Discovered Architecture Pattern}


% and conclude the general \textit{temporal modeling principle} based on searched results. As previous works \cite{xie2018rethinking, tran2018closer} stress several insights in resnet or inception based backbone including Top-heavy modeling strategy, R(2+1)D or S3D efficient efficient kernel, and temporal shift module , we revisit the temporal modeling pattern under the framework of mobilenet structure. 

We analyze the architecture pattern of these discovered architectures and give some discovered models in Fig. \ref{fig:visual}. While the overview of each model mainly follows the top-heavy building pattern which is consistent with that of inception-based model, a surprising finding is that the search algorithm tends not to choose the (2+1)D depthwise conv compared to the chance of others, conflicted with previous discussion on standard convolution. 
The reason is that (2+1)D standard conv saves large amount of actual FLOPs compared to 3D standard conv, while depthwise conv contributes little actual FLOPs in MobileNet structure. Take MobileNet-v2 with 8 input frames as a example, replacing the 2D depthwise conv with 3D depthwise conv only increases its FLOPs from 3.0G to 3.2G. However, same strategy on I3D will bring 4.1$\times$ additional FLOPs \cite{xie2018rethinking}. As R(2+1)D/S3D are designed to reduce the redundancy of standard 3D conv, it is no longer a charming choice under the framework of MobileNet, given the superior effectiveness of 3D depthwise convolution. 
% \zhicheng{This should be one of the most interesting part of the paper. I expect you discuss how arch searched on Kinetics and Something-something diff from each other. What is the connection between searched arch and search dataset? Ideally, you want to evaluate the transferability of arch, which is searched on kinetics, by benchmarking it on dataset something-something, or vice versa.}

\paragraph{Evaluation of Fairness Channel Selection} 
We further evaluate the effectiveness of channel fairness by analyzing both the performance of discovered architectures and the effectiveness of accuracy loss and FLOPs loss. To be more detailed, we provide the actual FLOPs of final discovered architectures under different weight of FLOPs loss. Comparing fair channel selection and unfair channel selection, fair selection introduces stronger relation between actual FLOPs number and the weight of FLOPs loss, while the the unfair one fails. This demonstrate the unfair channel selection rule distracts search process due to the unexpected updating rule of each channel candidates, results are shown in the supplementary.

% \zhicheng{If major results of fairness channel selection are in the supplement, you should start with "Discovered Architecture Pattern". }






% It is due to that depthwise convolution is a channel-separated operator which largely replys on the final pointwise convolution in each block to fuse the separable feature representation. In (2+1)D depthwise conv, the output feature maps of the first 2D spatial convolution need to forward pass the next 1D temporal convolution before they can be fused across each channel. Those differences take a main role that cause the different conclusion under different structures.

% 我们进一步研究了搜索出来的模型的pattern， 我们把搜索出来的模型的overview放在了figure3， 更多结果在supplementary。While top-heavy这个pattern也被我每的搜索算法发现了（前人也发现了）， 一个惊人的发现是，前人认为（2+1）D 在standard conv很work，我们发现当我们把（2+1）D应用在mobilenet（depthwise）上时，search算法大部分情况不会选（2+1）（depthwise）。原因在于，standard conv里不同的channel本身就有信息交互，但是depthwise非常依赖最后一个pointwise把feature融合起来，如果换成（2+1）D，第一个2D还是要等到第二个1D做完才能融合feature，这和原有的（2+1）D就不太一样了











%主要是和TVN比我们的search space完全不一样，我觉得是两个不同的框架下，我们更像和X3D一个框架，而X3D完全是基于手动grid search的" 之前的基于standardconv的work一致认为（2+1）D或者TSM是很efficient的kernel，但是我们的search算法大部分情况不喜欢选择这两个kernel，原因在于，standard conv里不同的channel本身就有信息交互，但是depthwise非常依赖最后一个pointwise把feature融合起来，如果换成（2+1）D，第一个2D还是要等到第二个1D做完才能feature融合，这和原有的（2+1）D就不太一样了，TSM同理，TSM也依赖于pointwise feature融合，我们的search算法几乎不选TSM，偶尔选一个

==> tex/5_experiment.tex <==
\section{Experiments}

\input{tex/5_1_implementations}

% \input{tex/5_2_setting}

\input{tex/5_2_ablation}

% \input{tex/5_3_fairness_filter_number_selection}

% \input{tex/5_4_search_in_full_space}

\input{tex/5_5_comparison_sota}
% \vspace{-5pt}
\input{tex/5_6_understand_autox3d}

==> tex/backup_fairness_filter_number_selection.tex <==


\subsection{Fairness-Aware Search of Filter Number}
\label{sec:exp_fairness_filter_number}

In Section~\ref{sec:fair_channel_selection}, we proposed fairness-aware search of filter number to ensure that the weights, which are shared by the choices of filter number, for each convolutional filter are updated with a fair chance at the beginning stage of the search. To study the importance of such fairness, we search for the architecture with the vanilla channel masking, where weights of the convolutional filters in the lower rank are more frequently updated. 
%We firstly analyze the supernet accuracy curve in the search stage, as shown in \textcolor{red}{xxx}. Thanks to the help of fair channel selection strategy, each activated sub-network is updated with the same frequency and can be fairly evaluated thus the accuracy curve is more stable. The network FLOPs of the vanilla channel masking quickly collapse to a small value, which we hypothesis this is due to the unbalanced on channels.
We analyze the searched architecture FLOPs in Fig. \ref{fig:flops_curve}. We conduct two searching experiments that one with the naive channel selection mechanism and the other one with our proposed fair channel selection. Other hyper-parameters are kept identical. We only search for the output channel and expansion ratio in those experiments. Thanks to the help of fair channel selection mechanism, each activated sub-network is updated with similar frequency and can be fairly evaluated, thus prevent the tendency of collapsing to select the well-updated small channel in the naive channel selection mechanism. We can observe the curve of FLOPs cost term of naive channel selection mechanism quickly collapse to zero, while ours is approaching to the target FLOPs steadily. 
%We found that the FLOPs cost term of the one with the naive channel selection mechanism collapse more quickly than the one with our fiar channel selection mechanism.
% We find the performance of searched results will generally decrease around $0.5\%$. %, details will be shown in the supplementary.
\begin{figure}[t!]
    \centering
\includegraphics[width=\linewidth]{figs/flops_curve.png}   
\caption{\textbf{FLOPs during searching.} For each epoch (x-axis), we derive the most probable architecture and measure its FLOPs (y-axis).}
    \label{fig:flops_curve}
\end{figure}

The accuracy and FLOPs of the searched architectures are presented in Tab. \ref{tab:cost}. The architecture searched with the naive channel selection mechanism has much lower FLOPs than the target FLOPs, while the FLOPs of the architecture searched with fair channel selection is on par with the target FLOPs. Also, the architecture searched with our proposed achieves much better video accuracy than the naive channel selection method ($70.5\%$ vs $73.1\%$).
\begin{table}[t!]
\centering
\resizebox{\linewidth}{!}{
  \begin{tabular}{l|c|c|c}
  \toprule
  \multirow{2}{*}{Search Strategy} & Target & Discovered  & Accuracy (\%) \\ 
   & FLOPs (G) & FLOPs (G) & Top-1 \\\specialrule{.1em}{.1em}{.1em}
  Naive Channel Selection & \multirow{2}{*}{2.0} & 1.7\textcolor{purple}{($-$\textbf{0.3})} & 70.5 \textcolor{purple}{($-$\textbf{2.6})} \\
  Fair Channel Selection (\textbf{ours}) &  & \textbf{2.0} & \textbf{73.1}  \\
  \bottomrule
  \end{tabular}
}
  \caption{\textbf{Architecture search with different channel selection mechanism.}}
\label{tab:cost}
\end{table}


==> tex/backup_search_glore.tex <==


\subsection{Searching for Attention Block}
% The placement location of attention blocks usually plays a significant role in the accuracy improvement of network. 
\begin{table}[t!]
% \vspace{-0.6cm}
\centering
% \small
% \tiny
% \scriptsize
\resizebox{\linewidth}{!}{

  \begin{tabular}{c|cccc|c|c|c}
  \toprule
     \multirow{2}{*}{Model} &  \multicolumn{4}{c}{Attention location}  & Params & FLOPS & \multicolumn{1}{c}{Accuracy ($\%$)} \\
    & S1 & S2 & S3 & S4 & (M) & (G) & Top-1 \\
    \specialrule{.1em}{.1em}{.1em}
    X3D-S  & - & - & - & - & 3.4 & 1.96 & 72.9  \\ \hline
     \multirow{4}{*}{Manual}  & 2 & - & - & -  &  &  & 72.6 \textcolor{purple}{(\textbf{$-$0.3})} \\
     & - & 2 & - & - &  &   & 73.0 \textcolor{c_green}{(\textbf{$+$0.1})} \\
     & - & - & 2 & - &  &   & 72.8 \textcolor{purple}{(\textbf{$-$0.1})} \\
     & - & - & 2 &  3 &  &   &  73.0 \textcolor{c_green}{(\textbf{$+$0.1})} \\ \hline
    Automatic & \multicolumn{4}{c}{Searched}   &  &   &  \textbf{73.3} \textcolor{c_green}{(\textbf{$+$0.4})}  \\
\bottomrule
% \specialrule{.1em}{.05em}{.05em}

  \end{tabular}
}
\caption{\textbf{Ablation in attention block insertion location}. The number $k$ under column S$n$ denotes $k$ attention blocks are uniformly placed in stage $n$. 
%\textit{VG} and \textit{DG} denotes vanilla GloRe block and Dual-GCN GloRe block, respectively. 
}
\label{tab:search_attention}
\end{table}



In the original GloRe paper\cite{glore}, 2 and 3 GloRe blocks are placed in stage 3 and stage 4 of the network respectively. We argue that such placement arrangement might not be the optimal setting. In this section, we adopt X3D-S as the baseline network, and only search for the placement locations of attention blocks. We also manually insert attention blocks into the network to create some manual-designed baselines. The configuration and results are shown in Tab. \ref{tab:search_attention}. Surprisingly, we observe that models with different attention locations perform quite differently. Improper insertion locations might even hurt the network performance. For example, inserting two GloRe in stage 1 brings inferior performance compared to X3D-S (\textcolor{red}{xx} vs $72.9\%$). We also find that the searched one brings better performance (\textcolor{red}{xx} vs $72.9\%$). Those experiments firmly demonstrate that the placement location of attention blocks is worth to be searched.



==> tex/broader_impact.tex <==

\section*{Broader Impact}
This work will inspire the human to better adopt artificial intelligence (AI) as a useful tool to improve our life. Since there is an increasing number of people uploading and watching videos in the Internet, it is an important topic about how we improve the user experiences in video websites. As a typical example, there are more than $10^5$ hours videos uploaded to YouTube in a day, and those need to be efficiently and effectively processed for recommendation system. The computer vision community has been working for decades to study diverse video analysis problem such as action recognition/understanding. The majority of latest video recognition models are computationally heavy, often using deeper/wider networks and high space-time resolution. Those expensive models turn impractical for nearly real-time or low-latency applications in mobile vision. To this end, successful design knowledge and building blocks for efficient image recognition models have been transplanted into video models too, including R(2+1)D \cite{tran2018closer}, TSM\cite{lin2019tsm}, MixTConv\cite{shan2020mixtconv}, and Video Shuffle Network\cite{ma2019learning}.

In this work, we propose an automatics algorithm to build the ultra-efficient video models. We take steps further towards the direction of extremely light-weight and efficient video recognition models. The goal is fundamentally challenging as it needs to combine the following two: (1) exploring the temporal-spatial feature patterns and their fusion across the network layers; and (2) integrating the variety of efficient network modules and other design options into the network. 
% The complicacy is further amplified by the model training workload on large-scale video recognition datasets. Such a daunting goal makes it no longer feasible to proceed with manual trial-and-errors.

Besides the benefits of video understanding itself, another goal of this work is to save energy and reduce carbon dioxide ($CO^2$) emissions which helps prevent greenhouse effect. As previous works \cite{feichtenhofer2020x3d, xie2018rethinking} spend much time on designing effective hand-crafted model, or use a computationally expensive way to search the diverse architectures (E.g. RL \cite{ryoo2019assemblenet}, Evolution \cite{piergiovanni2019tiny}), the design and search cost is extremely large. We firstly introduce a differentiable search algorithm to enables the block-type, channel numbers, expansion ratios, and input frames to be completely search. The search cost is largely reduced thanks to the weight sharing strategy and the searched architecture is both efficient and effective.

Despite the advantages of Auto-X3D, one potential concern is the user privacy security. Since deep learning method typically required gigantic data for training, the ill-use of user data may cause privacy violation. We would encourage the company to properly adopt automatic video analysis tool on their application and take care of the user privacy.

==> tex/ignore_5_3_search_backbone.tex <==
\subsection{Searching For Backbone w/o Attention Blocks}
\label{sec:search_backbone}

Our design space allows variable choices of block micro-architecture, filter number, expansion rate and attention blocks at different depth of the model. In contrast, the X3D~\cite{x3d} models not only use uniform micro-architecture, heuristic choices of filter number and constant expansion rate, but also lack the use of attention blocks as in our design space. In the first study where our focus is to fairly compare our searched models with the X3D models, we adopt a reduced design space where attention blocks are not used. Equivalently, that means in the macro-architecture of our space (Table~\ref{tab:macro-arch}), we do not add any attention block after each MBConv-3D block group.

We call our model searched in this reduced space as \autoxthreedS. During architecture evaluation, when we use an input size $T\times S^2 = 16\times224^2$, which is larger than input size $13\times160^2$ during architecture search, but keep the architecture unchanged, the model is called s as \autoxthreedM, following the convention in X3D. The results are shown in Table~\ref{tab:search_backbone}. By searching the block-type, filter number, and expansion ratio, \autoxthreedS achieves \textcolor{red}{xxx} accuracy and outperforms the hand-crafted X3D-S models by \textcolor{red}{xxx}. Meanwhile, \autoxthreedM is \textcolor{red}{xxx} higher than X3D-M with nearly the same FLOPs cost.

% zhicheng: add a dummy box to take the space which is expected to include discussions on the results in table tab:search_backbone
% \begin{solutionorbox}
% \vspace{4cm}
% \end{solutionorbox}

\begin{table}[t]
% \vspace{-0.6cm}
\centering
% \small
% \tiny
% \scriptsize
\resizebox{0.4\textwidth}{!}{

  \begin{tabular}{c|c|c|cc}
       \multirow{2}{*}{Model} & Params & FLOPS & \multicolumn{2}{c}{Accuracy ($\%$)} \\
       &  (M) & (G) & Top-1 & Top-5 \\
    \specialrule{.15em}{.1em}{.1em}
    
    X3D-S &  3.76 & 1.96  & 72.1* & \\
    \autoxthreedS   & 3.82* & 1.95*  & 72.9*  & \\ \hline
    X3D-M &  3.76 & 4.73  & 74.5* &  \\
    \autoxthreedM   & 3.82* & 4.76*  & 75.3*  &  \\

% \specialrule{.1em}{.05em}{.05em}

  \end{tabular}
}
\caption{\textbf{Comparisons to X3D models}. We evaluate them on Kinetics, and results of 10-Center testing are reported. }
\label{tab:search_backbone}
\end{table}

==> tex/ignore_5_4_search_in_full_space.tex <==
\subsection{Searching in the Full \autoxthreed Space}
\label{sec:exp_search_attention_blocks}

 Attention mechanism \cite{glore,nonlocal_block} has been demonstrated for its strong performance on both image and video benchmark. However, the poor efficiency of non-local block raises a major concern when applying on efficient architecture design. We evaluate the performance of both non-local unit and global reasoning unit on the ultra-efficient backbone X3D. As shown in Table. \ref{tab:search_in_full_space}, inserting different global reasnoning unit on different postion (from shadow to deep) mostly achieves a impressive improvement with few FLOPs cost, while non-local block costs much larger FLOPs in the early stage. This demonstrates the effectiveness and efficiency of global reasoning unit \cite{glore} and further motivate us to apply automatic search in terms of the block type and inserting position for global reasnong unit. Therefore, we search architectures in the full \autoxthreed space, where we jointly search the choices of block micro-architecture, filter number, expansion rate and attention block type for individual MBConv-3D block groups. The searched models from the full space are called as \autoxthreedSplus model. 

% Compared with the searched \autoxthreedS models in Section~\ref{sec:search_backbone}, attention blocks of the searched type are added to each block group in \autoxthreedSplus model. To highlight the importance of searching attention block types, we also build a strong baseline by manually inserting GloRe blocks to \autoxthreedS models. The results are shown in Table~\ref{tab:search_in_full_space}.

% \zhicheng{add discussions on the results in Table~\ref{tab:search_in_full_space}}.



% zhicheng: add a dummy box to take the space which is expected to include discussions on the results of searching attention blocks


==> tex/old_5_3_external_exp.tex <==
\subsection{Comparison with State-of-the-Art Models}


\begin{table*}[!t]
% \vspace{-0.8cm}
\centering
{\small
\resizebox{0.9\linewidth}{!}{
\setlength{\tabcolsep}{0.9mm}{
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
    % \toprule
    Model & Pretrain & Top-1 ($\%$) & Top-5 ($\%$) & \# Frames & GFLOPs$\times$ views & #Param (M)\\
  \specialrule{.15em}{.1em}{.1em}      
    I3D \cite{carreira2017quo} & ImgNet & 71.1 & 90.3 & 64 & 108 $\times$ N/A & 12.0 \\
    Two-Stream I3D \cite{carreira2017quo} & ImgNet  & 75.7 &  & 64 & 216 $\times$ N/A & 25.0 \\
    MF-Net \cite{chen2018multi} & ImgNet  & 72.8 & 90.4 & 16 & 11.1 $\times$ 50 & 8.0 \\
    TSM R50 \cite{lin2019tsm} & ImgNet  & 74.7 & N/A & 16 & 65 $\times$ 10 & 24.3 \\
    S3D-G \cite{xie2018rethinking} & - & 74.7 & N/A & 64 & 71.0 $\times$ N/A & N/A \\
    
    % \midrule
    
    Two-Stream I3D \cite{carreira2017quo} & - & 71.6 & 90.0 & 64 & 216 $\times$ N/A & 25.0 \\
    R(2+1)D \cite{tran2018closer} & - & 72.0 & 90.0 & 32 & 152 $\times$ 115 & 63.6 \\
    Two-Stream R(2+1)D \cite{tran2018closer} & - & 73.9 & 90.9 & 32 & 304 $\times$ 115 & 127 \\
    % ip-CSN-50 \cite{tran2019video} & - & 70.8 & - & 8 & 11.9 $\times$ 30 & 14.3M \\
    % ip-CSN-101 \cite{tran2019video} & - & 71.8 & - & 8 & 15.9 $\times$ 30 & 24.5M \\
    % SlowFast 4×16, R50 \cite{feichtenhofer2019slowfast} & - & 75.6 & 92.1 & - & 36.1 $\times$ 30 & 34.4M &\\
    % SlowFast 8×8, R101 \cite{feichtenhofer2019slowfast} & - & 77.9 & 93.2 & 84.2 & 106 $\times$ 30 & 53.7M &\\
    % SlowFast 8×8, R101+NL \cite{feichtenhofer2019slowfast} & - & 78.7 & 93.5 & 84.9 & 116 $\times$ 30 & 59.9M &\\
    % SlowFast 16×8, R101+NL \cite{feichtenhofer2019slowfast} & - & 79.8 & 93.9 & 85.7 & 234 $\times$ 30 & 59.9M &\\
    % X3D-L \cite{feichtenhofer2020x3d} & - & 77.5 & 92.9 & 83.8 & 24.8 $\times$ 30 & 6.1M &\\
    % X3D-XL \cite{feichtenhofer2020x3d} & - & 79.1 & 93.9 & 85.3 & 48.4 $\times$ 30 & 11.0M &\\
    % X3D-XXL \cite{feichtenhofer2020x3d} & - & 80.4 & 94.6 & 86.7 & 194.1 $\times$ 30 & 20.3M &\\
    \midrule
    TSM Mb-V2 \cite{lin2019tsm} & ImgNet & 69.5 & - & 16 & 6.00 $\times$ N/A & 3.9 \\
    % MobileNetV2-3D$_{8F}$  & - & - & - & 8 & 3.25 $\times$ 30 & 4.4M \\
    X3D-M$_{8F}$ \cite{feichtenhofer2020x3d} (our impl.) \cite{feichtenhofer2020x3d} & - & 69.3 & 88.6 & 8 & 2.47 $\times$ 30 & 4.4 \\
    \textbf{Auto-X3D-k1} & - & \textbf{70.7} & \textbf{89.4} & 8 & 2.50 $\times$ 30 & 6.0 \\
    \midrule
    MobileNetV2-3D (our impl.)  & - & 71.2 & 90.1 & 16 & 6.50 $\times$ 30 & 4.4 \\
    EfficientNetB3-3D from \cite{feichtenhofer2020x3d}  & - & 72.4 & 89.6 & 16 & 6.91 $\times$ 30 & 8.2 \\
    X3D-M$_{16F}$ \cite{feichtenhofer2020x3d} (our impl.\footnotemark) & - & 72.5 & 90.8 & 16 & 4.92 $\times$ 30 & 4.4 \\
    \textbf{Auto-X3D-k2} & - & \textbf{73.7} & \textbf{91.7} & 16 & 4.97 $\times$ 30 & 6.6 \\ 
    % \midrule
    % EfficientNetB4-3D from \cite{feichtenhofer2020x3d}  & - & 74.5 & 90.6 & 16 & 23.8 $\times$ 30 & 12.2M \\
    % \textbf{Auto-X3D-k3} & - & - &  & 16 & & \\ 
    \bottomrule
    \end{tabular}
    }
  }
}
\caption{\textbf{Comparisons to the state-of-the-art on Kinetics-400 dataset}. We use (GFLOPs $\times$ views) to represents inference cost $\times$ number of views). For evaluation, we uniformly sample 10 clips, and take 3 spatial croppings (i.e. Left, Center, and Right) per clip, and average the 30-view predictions.}
\label{table:Kinetics}
\end{table*}


\begin{table*}[t!]
\centering

\centering
{\small
\resizebox{0.95\linewidth}{!}{
\setlength{\tabcolsep}{0.9mm}{
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
    % \toprule
    Model & Backbone & Pretrain &  Top-1 ($\%$) & Top-5 ($\%$) & \# Frames & GFLOPs & #Param (M)\\
  \specialrule{.15em}{.1em}{.1em}      
    TSN \cite{zhou2018temporal}  & BNInception & ImgNet & 19.5 & - & 8 & 16 & 10.7 \\
    TSN from \cite{lin2019tsm}  & ResNet-50 & ImgNet & 19.7 & 46.6 & 8 & 33 & 10.7 \\
    TRN-Multiscale \cite{zhou2018temporal} & BNInception & ImgNet & 34.4 & - & 8 & 16 & 18.3 \\
    TRN-Multiscale from \cite{lin2019tsm} & ResNet-50 & ImgNet & 38.9 & 68.1 & 8 & 16 & 31.8 \\
    TSM \cite{lin2019tsm} & ResNet-50 & ImgNet & 45.6 & 74.2 & 16 & 33 & 24.3 \\
    ECO_{8F} \cite{zolfaghari2018eco} & BNInception+R3D-18 & - & 39.6 & - & 8 & 32 & 47.5 \\
    ECO_{16F} \cite{zolfaghari2018eco} & BNInception+R3D-18 & - & 41.4 & - & 16 & 32 & 47.5 \\
    % I2D \cite{xie2018rethinking} & Inception & - & 34.4 & 69.0 & 64 & & \\
    % I3D \cite{xie2018rethinking} & Inception & - & 45.8 & 76.5 & 64 & 108 & 12.06M\\
    I3D from \cite{wang2018videos} & R3D-50 & - & 41.6 & - & 32 & 153 & 28.0 \\
    % S3D \cite{xie2018rethinking} & Inception & - & 47.3 & 78.1 & 64 & 66 & 8.77M\\
    % S3D-G\cite{xie2018rethinking} & Inception & - & 48.2 & 78.7 & 64 & 71.38 & \\
    Non-local I3D from \cite{wang2018videos} & R3D-50 & - & 44.4 & 76.0 & 32 & 168 & 35.3 \\
    X3D-M$_{16F}$ \cite{feichtenhofer2020x3d} (our impl.) & MobileNet & - & 45.0 & 76.1 & 16 & 4.9 & 4.4 \\
    \textbf{Auto-X3D-k3} & MobileNet & - & \textbf{45.7} & \textbf{76.1} & 16 & 4.9 & 6.1 \\
    \bottomrule
    \end{tabular}
    }
  }
}
\caption{\textbf{Comparisons to the state-of-the-art on Something-Something-V1}. By default, we adopt uniform-sampling, which firstly divides the video sequence into $n$ uniform segments and then picks a random frame from each segment as the input frame. }
% \zhicheng{explain what is uniform sampling}.
\label{table:sthsthv1}
\end{table*}

% \footnotetext[2]{The original TVN paper \cite{piergiovanni2019tiny} reported no results on those benchmarks. Despite our best efforts to reproduce their methods and implement on the two datasets, their evolutionary algorithms were found to be ineffective in our experiments, whose results appear to be not reasonably competitive in Tables 2 and 3. We would be keen to include TVN into our comparison once their open-source implementations become available.}



We mainly follow the comparison convention of X3D \cite{feichtenhofer2020x3d} on popular large-scale benchmarks, and compare the performance of our Auto-X3D with current state-of-the-art efficient architectures\footnotemark . 
% We firstly conduct experiments on Kinetics-400 dataset  \cite{carreira2017quo}, details are shown in Table. \ref{table:Kinetics}. 
Top-1 accuracy as well as FLOPS are reported on Kinetics-400 dataset. We divide the models into three categories according to their FLOPs, details are shown in Table \ref{table:Kinetics}. The first group includes previous high-performance yet inefficient methods. Those methods either cost more FLOPs and parameters compared to ours, or get worse performance. In the second group, Auto-X3D-K1 achieves 70.7\% accuracy, better than TSM with mobilenet backbone (+1.2\%) and X3D-M$_{8F}$ (+1.4\%). Regarding FLOPs, Auto-X3D-k1 is 2.4$\times$ smaller than TSM with mobilnet backbone and costs comparable FLOPs compared to X3D-M$_{8F}$. In the third group, we evaluate a larger searched results named Auto-X3D-k2, it achieves 73.6\% accuracy and largely outperforms MobileNetV2-3D$_{16F}$ (2.5\%) and EfficienNet-B3-3D (1.3 \%), with 1.30$\times$ and 1.39 $\times$ smaller FLOPs respectively. Compared to X3D-M$_{16F}$, Auto-X3D-k2 reaches 1.2\% higher accuracy with similar FLOPS cost. 
% In the fourth group, to evaluate the scalability of searched architectures, we scale up the Auto-X3D-k2 by increasing its depth to 1.46$\times$ layer. 

In addition, We further apply the searched architecture on Kinetics to train on Something-something v1 dataset in order to demonstrate the generalization of discovered architectures. We include current state-of-the-art methods in Table \ref{table:sthsthv1}. Auto-X3D-k3 outperforms Non-local I3D (1,3\%) and TSM R50 (0.1\%) with much less FLOPs. Moreover, Auto-X3D-k3 is 0.7\% higher than X3D-M$_{16F}$ with nearly same FLOPs. These impressive results verify both the high performance and transferability of our NAS framework.













==> tex/old_5_4_ablation_study.tex <==
\subsection{Ablation Studies}
\begin{figure*}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}} 
 \includegraphics[width=\linewidth]{figure/Visualize.pdf}
\end{center}
% \vspace{-1em}
   \caption{\textbf{Discovered architectures}. The length of each block represents the expansion ratio and the filter number is marked inside the block. We find that the bottom-layers mostly choose spatial operator while the top-layers mostly choose temporal operators. This finding is consistent with previous conclusion on inception-based architectures \cite{xie2018rethinking}.}
%   \zhicheng{The caption is weak, and the figure is too simple now. Can you encode the width/expansion rate in the architecture as well? How does the searched arch resonate the top-heavy/bottom-heavy findings in hand-crafted models? Can you discuss a bit in caption?} 
\label{fig:visual}
\end{figure*}

\paragraph{Discovered Architecture Pattern}


% and conclude the general \textit{temporal modeling principle} based on searched results. As previous works \cite{xie2018rethinking, tran2018closer} stress several insights in resnet or inception based backbone including Top-heavy modeling strategy, R(2+1)D or S3D efficient efficient kernel, and temporal shift module , we revisit the temporal modeling pattern under the framework of mobilenet structure. 

We analyze the architecture pattern of these discovered architectures and give some discovered models in Fig. \ref{fig:visual}. While the overview of each model mainly follows the top-heavy building pattern which is consistent with that of inception-based model, a surprising finding is that the search algorithm tends not to choose the (2+1)D depthwise conv compared to the chance of others, conflicted with previous discussion on standard convolution. 
The reason is that (2+1)D standard conv saves large amount of actual FLOPs compared to 3D standard conv, while depthwise conv contributes little actual FLOPs in MobileNet structure. Take MobileNet-v2 with 8 input frames as a example, replacing the 2D depthwise conv with 3D depthwise conv only increases its FLOPs from 3.0G to 3.2G. However, same strategy on I3D will bring 4.1$\times$ additional FLOPs \cite{xie2018rethinking}. As R(2+1)D/S3D are designed to reduce the redundancy of standard 3D conv, it is no longer a charming choice under the framework of MobileNet, given the superior effectiveness of 3D depthwise convolution. 
% \zhicheng{This should be one of the most interesting part of the paper. I expect you discuss how arch searched on Kinetics and Something-something diff from each other. What is the connection between searched arch and search dataset? Ideally, you want to evaluate the transferability of arch, which is searched on kinetics, by benchmarking it on dataset something-something, or vice versa.}

\paragraph{Evaluation of Fairness Channel Selection} 
We further evaluate the effectiveness of channel fairness by analyzing both the performance of discovered architectures and the effectiveness of accuracy loss and FLOPs loss. To be more detailed, we provide the actual FLOPs of final discovered architectures under different weight of FLOPs loss. Comparing fair channel selection and unfair channel selection, fair selection introduces stronger relation between actual FLOPs number and the weight of FLOPs loss, while the the unfair one fails. This demonstrate the unfair channel selection rule distracts search process due to the unexpected updating rule of each channel candidates, results are shown in the supplementary.

% \zhicheng{If major results of fairness channel selection are in the supplement, you should start with "Discovered Architecture Pattern". }






% It is due to that depthwise convolution is a channel-separated operator which largely replys on the final pointwise convolution in each block to fuse the separable feature representation. In (2+1)D depthwise conv, the output feature maps of the first 2D spatial convolution need to forward pass the next 1D temporal convolution before they can be fused across each channel. Those differences take a main role that cause the different conclusion under different structures.

% 我们进一步研究了搜索出来的模型的pattern， 我们把搜索出来的模型的overview放在了figure3， 更多结果在supplementary。While top-heavy这个pattern也被我每的搜索算法发现了（前人也发现了）， 一个惊人的发现是，前人认为（2+1）D 在standard conv很work，我们发现当我们把（2+1）D应用在mobilenet（depthwise）上时，search算法大部分情况不会选（2+1）（depthwise）。原因在于，standard conv里不同的channel本身就有信息交互，但是depthwise非常依赖最后一个pointwise把feature融合起来，如果换成（2+1）D，第一个2D还是要等到第二个1D做完才能融合feature，这和原有的（2+1）D就不太一样了











%主要是和TVN比我们的search space完全不一样，我觉得是两个不同的框架下，我们更像和X3D一个框架，而X3D完全是基于手动grid search的" 之前的基于standardconv的work一致认为（2+1）D或者TSM是很efficient的kernel，但是我们的search算法大部分情况不喜欢选择这两个kernel，原因在于，standard conv里不同的channel本身就有信息交互，但是depthwise非常依赖最后一个pointwise把feature融合起来，如果换成（2+1）D，第一个2D还是要等到第二个1D做完才能feature融合，这和原有的（2+1）D就不太一样了，TSM同理，TSM也依赖于pointwise feature融合，我们的search算法几乎不选TSM，偶尔选一个
